Facebook Ads Monitor: An Independent Auditing System for Political Ads on Facebook

The 2016 United States presidential election was marked by the abuse of targeted advertising on Facebook. Concerned with the risk of the same kind of abuse to happen in the 2018 Brazilian elections, we designed and deployed an independent auditing system to monitor political ads on Facebook in Brazil. To do that we first adapted a browser plugin to gather ads from the timeline of volunteers using Facebook. We managed to convince more than 2000 volunteers to help our project and install our tool. Then, we use a Convolution Neural Network (CNN) to detect political Facebook ads using word embeddings. To evaluate our approach, we manually label a data collection of 10k ads as political or non-political and then we provide an in-depth evaluation of proposed approach for identifying political ads by comparing it with classic supervised machine learning methods. Finally, we deployed a real system that shows the ads identified as related to politics. We noticed that not all political ads we detected were present in the Facebook Ad Library for political ads. Our results emphasize the importance of enforcement mechanisms for declaring political ads and the need for independent auditing platforms.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> WWW-CONF 2/1-introduction.tex <==
\section{Introduction}

%\oana{I think the point that we should make in this paper is that we need independent auditing platforms for political ads because it is not a good idea to just rely on Facebook to do this;  we also show that this is feasible}

%\oana{we need to talk about propublica as well}

%\oana{need to talk about Facebook archive}

%\oana{
%The paper tells the story of our effort to deploy a system to identify the political ads and the impact it had
%


%\oana{we need to get this introduction very factual and do not assign blame, do not overclaim. Also we need to check if all the events we talk about actually happened the way we describe them}
%\oana{i tried to do a first pass and be more factual}

	
% Elections in USA and Target advertising


%The Facebook advertising platform was abused before the US presidential elections
The 2016 United States presidential election was marked by an information war that took place into different social media platforms~\cite{badawy2018analyzing,lima2018@asonam}. In particular, the election was marked by the abuse of targeted advertising on Facebook;
%which is meant to improve the efficiency of matching advertisers to their customers but can also be abused by malicious political campaigns to spread false stories. 
a group of Russian citizens and companies were indicted by U.S. authorities for trying to influence the 2016 US election through the Facebook Ad Platform~\cite{russian-ads,cnnrussian}. A recent study characterized a set of ads released by the house of representatives posted by the Russian company named Internet Research Agency (IRA)~\cite{ribeiro2019@fat}. Their findings show that these ads received a click-through rate about 10 times higher than the one for typical ads in Facebook, that ads were ran along two years and not only during the 2016 election, and that the content of these ads was on polarizing topics (e.g., immigration, race-based policing), usually targeting vulnerable sub-populations. 
%
The case of the IRA ads clearly raised numerous concerns about external interference in elections through targeting advertising.  Beyond that, it showed how an ad platform could be used for posting illicit political ads targeting people susceptible to false stories, stoke grievances, and incite social conflict. In other words, a platform of this kind could be abused to engineer polarization in a country, which could end up favoring a political campaign. 

%As an answer to these new threats, Facebook implemented several measures. On May 24, 2018, it changed its ToS policy to allow the launching of political ads only by advertisers that reside in the same country with the people targeted (this requirement does not apply to non-political ads). Additionally, Facebook launched an ad archive to show the ``active campaigns'' of advertisers that send political ads that are accessible from their corresponding Facebook Pages. This service ran as a test pilot in Canada, before it was launched for the Brazilian elections, June 28 2018. This service not only allows people to see all the ads deemed \emph{political}, but also provides information on how much money was spent on them. \thanos{I have in the comments in the next paragraph the original text, because it was not clear, can someone verify that the new text is correct} 

As an answer to these new threats, Facebook implemented several countermeasures. On May 24, 2018, Facebook changed its ToS policy to allow the launching of political ads only by advertisers that reside in the same country with the people targeted (this requirement does not apply to non-political ads)~\cite{tos_change_facebook}. Also, all election-related ads must be clearly labeled as such, including a “Paid for by” disclosure from the advertiser at the top of the ad.
On June 28, 2018, Facebook launched a page to show the ``active campaigns'' of advertisers that send political ads that are accessible from their corresponding Facebook Pages~\cite{facebook_adarchive_lached} (this service was a test pilot only available in Canada before the Brazilian elections between Aug. 16 -- Oct. 28, 2018). 
Finally, in June 2018 Facebook launched the Facebook Ad Library~\cite{facebook_ad_archive_launched, facebook_ad_archive}, a service that allows people to see all the ads declared as \emph{political} by the  advertisers posting them  as well as information about who paid for the ad, the amount spent, the number of impressions delivered, and the audience. 
A few weeks after that, Facebook launched the Ad Library to Brazilian citizens~\cite{facebook_ad_archive_launched}. 
%\oana{ads deemed political by whom?}
%\oana{when was the brazilian archive launched?}

%\oana{Fabricio, can you check if the dates are correct and we  are describing these events properly?}
%\thanos{I am a bit confused with the timeline. Can someone that knows the timeline better make a pass? (and fix also the citations, I think we need one with the actual Facebook Ad Archive)} %However, during the Brazilian elections, only US researchers had access, and, after US the Brazil had access .%\footnote{While as of April 2019 there are more transparency mechanisms implemented by Facebook (which we will discuss later), this was the situation in August 2018.} 

%Why these measures are not enough:
%	- advertisers have to declare themselves on a voluntary base
%	- slush campaigns

While these measures were welcomed, many people including researchers, journalists and organisations pointed out that they are not sufficient~\cite{efective_ad_archive, mozillaadlibraryreport, cnnAdLibraryDontWork}.
\textit{First}, advertisers have to declare themselves, on a voluntary basis, whether they are sending political ads. %; and the interface does not offer information about past campaigns. 
This is problematic because dishonest political parties and presidential candidates can avoid scrutiny of their ad messages by not declaring them as political. \textit{Second}, beyond public opinion manipulation and spread of fake news, the Facebook ads platform can also be used for \emph{slush funds}~\cite{fabriciofolha}. Brazilian electoral law states that companies are prohibited to make donations to any political party or candidate during the election period. Currently, dishonest companies can spend an unlimited amount of undeclared money in favor of a political agenda through the Facebook ads platform~\cite{electoral_law}. 
%However, since only Facebook has information about who and how much was paid for ads, anyone, and potentially any company,
%Other reasons why current efforts by Facebook are not enough is that one needs to know the existence of advertisers in order to be able to check his ads and 
\textit{Third}, the Facebook Ad Library does not offer information regarding the targeting used by advertisers. A recent study found out that Facebook makes available to advertisers more than 240,000 interests that it has inferred about its users, such as ``Yoga'', ``Gluten-free'', or ``Adult Children of Alcoholics''~\cite{speicher-2018-targeted} . Combinations of these interests can result in uncontrollable ways of reaching very specific sub-populations vulnerable to specific messages. 

Advertisers of political content are supposed to both comply with the Facebook's Terms of Service as well as the election legislation in their respective countries.  
In October 2017, Brazilian authorities demanded that political figures that are advertising on Facebook political content along the electoral period, an established period near the elections, need to give information about their national identification numbers, namely CPF, for individuals, and CNPJ, for companies. Facebook responded by creating an interface that allows advertisers of political content to include disclosure information in their ads related to elections and also their CNPJs or CPFs (see Figure~\ref{fig:ad_anastasia}). However, Facebook we are unsure whether they deployed any enforcement mechanisms for tagging political ads that try to run without the right disclaimer in Brazil.


%We decided to deploy a system to detect political ads; what are the challenges
%	- we need collaborative platform because microtargeting
%	- allow users to search for political ads
%	- describe how it worked and what are the features
% 	- we need to monitor the targeting as well
Concerned by the eminent high potential misuse of Facebook ads and imminent risks to Brazilian electoral laws, we designed and deployed a system to monitor political ads on Facebook, named \admonitor\footnote{\url{https://www.eleicoessemfake.dcc.ufmg.br/anuncios}}\footnote{The extension has been forked from \url{adanalyst.mpi-sws.org}.}. 
%\url{http://150.164.1.202/ads/}}}. 
%The main challenge towards understanding the extent to which the Facebook ads platform can be abused, is that the targeted ads are only seen by the targeted users. Hence, 
Our tool is a Chrome and Firefox extension that users can install on their computers and that collects the ads users see when they check their Facebook timeline as well as the corresponding explanations from the ``Why am I seeing this ad?'' feature that reveals some information about the targeting used by the advertisers~\cite{Andreou19a}. Our tool is similar with the tools provided by ProPublica~\cite{propublicahome} and WhoTargetsMe~\cite{whotargetsme}, but it is customized for collecting and analyzing ads in Portuguese besides English.
%
In addition, we developed a web application that runs our political ad classifier and allows Brazilian authorities and citizens to monitor the Facebook ads that our browser extension has collected. The classifier calculates the political probability score for each ad we collect. Our web application has a search engine where anyone can search and perform filters over our data.  Our hope was that the detection of a single illegal ad is enough to incur strict penalties and, hopefully, to inhibit the proliferation of such ads. 
%\oana{link for the servie? is the service still working?}







%\update{While our main goal was to inhibit the weaponization of online targeted advertising to spread misinformation and opinion manipulation in the Brazilian elections, the deployment of this system enabled us to pinpoint limitations with current transparency solutions and discover opportunities in going forward. We sum up next both our academic and more societal contributions:} \oana{paragraph needs more wokr}



%Contributions and impact of this work
%	- societal: dissemination  with politicians and opinion articles  lead to changes in the laws	; 	- after this there were new lows implemented; facebook more mechanisms for Brazil
%	- algorithms: scientific -- algorithms to detect political ads; use tweets to detect political ads it is nice! cross-platform
%	- results:  many ads not captures show the need for multiple independent auditing authorities; compare with facebook archive;
%	- code: open source}

%\paragraph{Societal impact} 
%\change{The deployment of the system enabled us to pinpoint limitations with current transparency solutions and discover opportunities for improving the accountability of political ads. We sum up next both our academic and more societal contributions:}
%\oana{do not like yet this paragraph} \oana{maybe cut it? move it at the end?}

%\textbf{Reachout}: 
To disseminate the tool we wrote and published opinion articles on the media disclosing ways  in which online systems can be exploited to influence elections and what we can do about them\cite{fabriciofolha, nyt2018benevenuto}.  We also presented these threats in the Brazilian senate.\footnote{\url{https://www12.senado.leg.br/noticias/materias/2018/05/11/impacto-das-midias-sociais-para-o-legislativo-sera-discutido-em-seminario-no-senado}}\footnote{\url{https://www.youtube.com/watch?v=eGScrdi5hhU&t=3450s}} 
Our tool was installed by more than 2000 users, out of which 715 users actively used the tool along the election period, providing us all the ads they received while navigating on Facebook. This collaborative effort provided us with a dataset containing 239k ads from 40k advertisers along the period of March 14, 2018 to October 28, 2018. 


%Once the risks became clear and eminent, Brazilian authorities pushed Facebook to find solutions to these problems. Facebook responded by building a feature that allows users to view political ads on a page and their information about the party or political CNPJ (Brazilian tax id for companies) who paid for the ad, the amount spent, the number of impressions delivered, and the audience. According to Facebook, advertisers of political content during elections have now to include disclosure information in their ads related to elections.}
%\oana{is this precise? do we overclaim?@Fabricio, can you do a pass?}
%\oana{we should also talked that you were invited to the senate? and to talk with the president of the committee who organizes the election.}



\begin{figure}[t]
\includegraphics[width=1.0\columnwidth]{figures/sample_ad.png}
\caption{Example of an official political ad posted during the election period in Brazil.}
\label{fig:ad_anastasia}
\end{figure}






%\paragraph{Algorithm to detect political ads:} 
%\textbf{Evaluation of supervised learning methods to detect political ads}: 
We implemented several machine learning-based techniques for detecting political ads on Facebook. 
%Particularly, a Convolution Neural Network (CNN), previously proposedto detect political Facebook ads using word embeddings. 
We tested supervised classifiers such as Naive Bayes, Random Forest, Logistic Regression, SVM and Gradient Boosting as well as a recently proposed Convolution Neural Network (CNN) built to detect political tweets.
 To evaluate our algorithms we created a golden standard test collection with 20k ads labeled as political or non-political.\footnote{\label{dataset}Dataset and code available at \url{https://lig-membres.imag.fr/gogao/political_ads.html}.} Our results show that the CNN-based model is able to achieve an AUC of 98\% and  an accuracy of 94\% in a near balanced dataset or a 78\% true positive rate for a 1\% false positive rate.
 %while the Naive Bayes classifier achieves a 85\% true positive rate for a 1\% false positive rate.
%\oana{ it is a bit weird that in section 5 we use CNN instead of Naive Bayes because NB has a better accuracy}
%Oana we won of 4 machine learning with few data, with more data  \cite{chen_deep_learning} said we will beat any machine learning techniques with deep learning (CNN, LSTM, etc...). 


%We show that a Convolution Neural Network (CNN) our method outperforms classic supervised machine learning strategies such as the one implemented by ProPublica~\cite{propublica} and is quite effective with \update{$94\%$} of \emph{Macro-F1} and \update{$1.0\%$} of \emph{confidence interval}.

%While there are several works that propose algorithms to detect political content on Twitter, this is the first academic algorithm to detect political ads. 

%\paragraph{Ads Dataset:}


%In addition, we developed a web application that runs our political ad classifier and allows Brazilian authorities and citizens to monitor the Facebook ads that our browser extension has collected. The classifier calculates the political probability score for all ads in the database (\datasetBrazil). Our web application has a search engine where anyone can search and perform filters over the full \datasetBrazil. %For a given search query, it retrieves and exhibits the ads sorted by the probability calculated by the classifier in descending order.
%Our hope was that even though our sampled data is small in comparison with the entire set of ads running during electoral period,



%\paragraph{Evaluation of current transparency mechanisms:} 

%\textbf{Evaluation of current transparency mechanisms:} 

%\textbf{Independent Auditing System}:


We tested the CNN classifier over a dataset of 38k ads containing ads in Portuguese during the electoral period (August 16, 2018 to October 28, 2018), and we found 835 (approx 2\%) of the ads to be political. Even if we only have a small sample of ads running on the platform, our results show that there are many ads with political content that were detected by our algorithm and were not labeled as such on Facebook. %We identified a large set of political ads that are bypassing Facebook and potentially the Brazilian law. %Finally, we examined how well political ads are represented in the Facebook Ad Library by comparing the ads detected by our algorithm with the ads labeled as political in the Facebook Ad Library.  Only \update{10\%} of the ads we detected as political were labeled as such in the Facebook Ad Library. % \change{We identified a large set of political ads that are bypassing Facebook and potentially the Brazilian law. %This result emphasis the need of independent auditing systems for political ads in Facebook such as the one we have created. 
%While this result is undeniably worrying as there are Brazilian advertisers that did not declare their political ads, there is a positive side to it: we can exploit the ads labeled as political from compliant advertisers to build machine learning-based models that can detect other similar ads coming from advertisers that do not comply with the Facebook's ToS or electoral laws. %with a very high accuracy.  

%In this study we only tested machine learning-based models trained on ads in Portuguese and evaluated them only on ads during the 2018 Brazilian elections.  Assessing the accuracy of such techniques on ads in other languages and testing how well these techniques are adapting to future elections remains an open question. 

%\oana{I want for the reader to apreciate the beauty of having access to a recent, evolving, across country dataset of political ads comminf from compliant advertisers. Which allows us to build models that evolve with the election and the language,}

%\oana{need to talk about more precise things in the evaluation -- this should be the meat of the academic contributions} We do an in-depth characterization of these ads. 
%Later in May 28, 2018 Facebook started to offer an archive of all political ads on the platform \cite{facebook_adarchive_lached}.  Unfortunately, we noticed that not all political ads were tagged as such over the platform. Indeed our analysis shows that there are many ads that are missed by Facebook and detected by our algorithm. Section \ref{sec:results} presents a characterization of what ads our platform detects in comparison with those identified as political by Facebook.  

%\oana{need more precise numbers for this section}



Our study emphasize the importance of enforcement mechanisms for declaring political ads.  The big open questions, however, are (i) who is responsible for enforcing the election legislation?; and (ii) how can authorities be able to enforce laws if they do not have access to data?
While companies and politicians are debating how to regulate political ads \cite{twitter_ban_political_ad, microtargeting_europe}, we believe one potential solution could be independent auditing platforms such as ours that collect ads from volunteers and search for undeclared political ads. We show that it is feasible to build such a platform and have a positive impact in the real world.   Our auditing platform is online (\url{https://adanalyst.mpi-sws.org/}) and we plan to monitor other elections as well.  Furthermore, to facilitate the development of new auditing platforms, our code is open source and some parts of our data are public.\footref{dataset}%Multiple auditing systems can also make the whole ecosystem more robust to malicious advertisers that attempt to circumvent detection.






% \oana{not related with the rest; move to conclusion}

%As Facebook has no obligation of providing transparency about the ads run in their platform, this platform can be widely abused along political elections. \oana{not sure if this is true, lots of pressure on Facebook to do something about the ads on the platform}

%\oana{what were the steps taken in Brazil to avoid same thing happening}

%In this paper, we present  a system to provide transparency for political ads in Facebook. %Worried about the upcoming abuse of targeting advertising in the 2018 Brazilian elections, we designed, evaluated and deployed a real system to identify political ads along the Brazilian elections.
%
% Our effort consisted of three steps: 
%(1) \textit{Gathering Facebook Ads}. 
%We built a slightly modified version of \adanalyst  to allow the collection of Facebook ads from volunteers in Brazil. We call this version as \adanalystbr. Our project was discussed in many Brazilian news outlets and
%
%(2) \textit{Identifying Political Ads}.
%
%
%(3) \textit{Deploying and Evaluating a System}. We deployed our approach for detecting political ads in our dataset and allowed users to search for political ads posted along the 2018 Brazilian elections. 
%


%The 2016 United States presidential election called into question the belief in the Internet as an environment that, by its own open architecture, would act necessarily and always as a vehicle for inclusion, freedom and democratization of the physical world. However, in 2017, Russian citizens and companies were indicted by American authorities of influencing on the 2016 US election using the Facebook Ads Platform \cite{russian-ads,cnnrussian}. This fact brings up the political ads influence issue to peak of society's discussion.

%Thus, techniques to prevent or mitigate the side effects of misuse political ads on social networks are necessary. Indeed, Facebook recently implemented a mechanism where advertisers put their Brazilian tax id, in order to track all the money they are spending with ads. In addition, political advertisers have to tag their ads as \emph{political ads}. Advertisers that place political ads without tagging them and providing their tax id go against the law and could even go to jail.  On the other hand, malicious advertisers are always willing to break the law and spread misinformation through sponsored content on social networks. Thus, computational mechanisms are necessary to detect and warn authorities about illegal and suspicious ads. Some tools reflect this need already; ProPublica~\cite{propublica} is a crowdsourcing browser extension which gathers Facebook ads for the public to label them as political or non-political, and \adanalyst\footnote{All references that might de-anonymize the authors of this study have been redacted for the submission process.} is a browser extension that collects ads and investigates how the Facebook ads ecosystem works, how advertisers target users and makes the system more transparent to the users. 

%Still though, the challenge of gathering and identifying political ads is far from being solved\cite{grimmer_stewart_2013}. The main problem is that these ads mostly do not ask for votes directly, but instead try to influence political opinion by targeting controversial subjects that are clearly associated with the political agenda of a given candidate, such as gay rights, gun control, abortion, immigration and race.
%, with quite a few citing the names of candidates such as Hillary Clinton (Democrat) and Donald Trump (Republican).
%The ecosystem of Facebook Ads Platform is complex and gives advertisers a wide range of options to target users. Till \textit{et. al.}~\cite{speicher-2018-targeted} showed how it is possible in Facebook to spread opinions or perform discriminatory advertising without using sensitive attributes directly, but by leveraging other attributes that Facebook has inferred for users. Thus, political ads can spread content about hate speech, fake news or discrimination of minorities. %%speicher-2018-targeted - Till

%Beyond micro targeted advertising, malicious advertisers can pulverize tiny incomes in multiple fake accounts. This technique aims to make money tracking hard and avoid attracting authorities' attention. All money not declared to authorities during elections is called slush fund. Generally, this money is an advance payment to receive any bribe, contract, kickback or other illicit payment or benefit in violation of the law after elections. In short, Facebook ad platform does not provide any public interface for authorities, lawmakers, regulators, journalists or any civil society stakeholder to detect misuses of the platform. Thus, nobody knows how many ads are running for each time window.  Also, there is not any way to measure how many likes, shares, comments, targeted audience or interactions an ad received. Recently, a web search interface for political ads was deployed by Facebook, but it contains only a few information about these ads such as text, image or video, and it does not include any API~\cite{upturn}. Finally, automated political ad identification is a hard task due to language nuances. 

%Overall, we believe that, by providing an automated public system called \admonitor based on a machine learning approach, our work is a first step towards designing better techniques for ad identification issue. In this work, we propose a Convolution Neural Network (CNN) to detect political Facebook ads using word embeddings, as well as a complete methodology to label ads. We also compare it to other machine learning approaches such as Logistic Regression, Naive Bayes (MultinomialNB) and Gradient Boosting. Our best strategy has $88\%$ of \emph{Macro-F1} score. Additionally, we built a slightly modified version of \adanalyst to allow the collection of Facebook ads from contributors and we call this version as \adanalystbr, In total, 715 users installed and activated our tool. This collaborative effort proved to be fundamental for the success of our system.

The rest of the paper is organized as follows. Section~\ref{political_ads} provides the necessary background on the Brazilian election legislation and how the Facebook ad platform works. Section~\ref{sec:dataset} describes our dataset and data collection method. Section~\ref{sec:methodology} describes our algorithms for detecting political ads and Section~\ref{sec:results} describes the results and findings after deploying our system in the real-world. Finally, Section~\ref{related-work}, highlights our contributions in comparison with related studies. %Finally, we show our final considerations and next steps towards model improvements in Section \ref{sec:conclusion}. 

%After the commotion around the 2016 US Elections, Brazilian authorities were afraid of a new large scale misuse of political ads on Facebook during the Brazilian elections. Beyond public opinion manipulation and spreading fake news, the Facebook ads platform can also be used for slush funds, because in Brazil companies are prohibited to make donations to any political party or candidate. Concerned by this eminent high potential misuse of Facebook ads, our research leader wrote and published some opinion articles on the media about how candidates could exploit Brazilian electoral laws through the Facebook ads platform. The idea is simple: since only Facebook has information about who and how much was paid for ads, anyone, and potentially any company, could spend an unlimited amount of undeclared money in favor of a political agenda through the Facebook ads platform with no risks whatsoever. By the time of those articles, Facebook had no audit mechanism or transparency tool for preventing this to happen.


%After this opinion article, the Brazilian authorities started to worried about the possibilities pointed. Next, Facebook was asked how it would solve the issues mentioned. Then, the Facebook has built a feature allows users to view ads on a page and can view information about the party or political CNPJ (Brazilian tax id for companies), the amount spent, the number of impressions delivered, and the audience. According to Facebook advertisers will have to include a disclosure in their ads related to elections.












==> WWW-CONF 2/2-background.tex <==
\section{Background} \label{political_ads}


This section provides background on the Brazilian election and legal requirements for advertising political content, as well as how advertising on Facebook works, what are the platform's Terms of Service regarding political content, and transparency mechanisms provided. 
Note that there is a distinction between the legal requirements from state legislation that advertisers have to follow, and the requirements advertisers need to respect due to the ToS of Facebook.

\subsection{Brazilian Election Legislation} 

In Brazil elections occur every four years and are divided between national and local elections. In national elections, Brazilian citizens choose their president, governors, deputy-governors, state representatives, senators and congressmen in all 26 states and the Federal District. Local elections are for choosing mayors and councilors. 

%\update{Fabricio: Pedro, please review the following two paragraphs carefully}

The 2018 presidential elections in Brazil had two rounds. To win the election directly in the first round a candidate should have at least 50\% of the valid votes, which was not the case in 2018. The voting period for both rounds last only a single day. In 2018, the first round was in October 7 and the second round in October 28. From August 16 onward, \emph{electoral advertising}, such as rallies, caravans, distribution of graphic material and advertising on the Internet was permitted.

%For the 2018 elections, the Superior Electoral Court of Brazil stipulated that electoral propaganda on the Internet was only allowed from August 16 and obeying a well-defined set of rules.

%We call electoral period the established period that proceeds both voting days.  In the 2018 elections, it started on August 16 and ended in October 28. 


%The 2018 presidential elections in Brazil had two rounds. To win the election directly in the first round a candidate should have at least 50\% of valid votes, which was not the case for electing the president. The voting period for both rounds last only a single day. In 2018, the first round was in October 7 and the second round in October 28. We call electoral period the established period that proceeds both voting days.  In the 2018 elections, it started on August 16 and ended in October 28. 

For electoral advertisements on the Internet, Resolution No. 23,551 of the Superior Electoral Court of Brazil~\footnote{\url{http://www.justicaeleitoral.jus.br/arquivos/resolucao-23551-nova/rybena_pdf?file=http://www.justicaeleitoral.jus.br/arquivos/resolucao-23551-nova/at_download/file}} stipulated a series of rules in order to ensure greater transparency for campaign spending. For advertisements on social networks, such as on Facebook, chapter IV of the resolution stipulates that they can be made or edited by:
\begin{itemize}
    \item candidates, political parties or coalitions;
    \item any natural person (e.g. a bot or a fake profile \emph{is not} a natural person), \textit{as long as they do not pay for content promotion}. Meaning that they can only promote candidates through regular posts and not sponsored ads. 
\end{itemize}
In addition, any promoted content must contain, in a clear and legible form, the registration number in the National Register of Legal Entities (CNPJ)~\footnote{An identification number issued to Brazilian companies by the Department of Federal Revenue of Brazil.} or the registration number in the Register of Individuals (CPF)~\footnote{The Brazilian individual taxpayer registry identification.} of the responsible person, in addition to the expression \emph{``Electoral Advertising''} (in Portuguese: \emph{Propaganda Eleitoral}).

Also, Paragraph 4 of Article 23 of the resolution stipulates that the Internet application provider (e.g., Facebook) that allows paid political content to be promoted must clearly communicate this to its users. In compliance with this law, Facebook provides an interface for political agents to properly register their advertisements during the election period. Figure~\ref{fig:ad_anastasia} shows an example of a political ad properly promoted on Facebook using this interface. All the respective expenses with those ads needed to be declared to the Superior Electoral Court.

%The use of social media, as well as the use of targeted advertising, was allowed in the 2018 election. In this case, political ads posted during the electoral period are considered as \textit{electoral ads}, which need to follow a specific regulation.  First, they should explicitly say that the ad is an electoral ad. This could be done in the ad body text or by sharing it as an electoral ad, a new option in the Facebook interface available along that period. By sharing using this last option, the ad was accompanied by an ``Electoral ad'' tag (In Portuguese: \emph{Propaganda Eleitoral}) as we can see in the example in Figure~\ref{fig:ad_anastasia}.Second, the respective expenses with those ads needed to be declared to the Electoral Court. All candidates must put their Brazilian tax id in their electoral  ads (which is used in a similar way to the Social Security Number in the U.S). Another possibility is to use the tax id of the political party, when the political party was the responsible one for paying for the ad~\cite{electoral_law}. The election law also states that only politicians and political parties are allowed to post electoral ads. 
%More importantly, in Brazil, it is illegal to post electorial political ads in a 1-month period before the election. 

%

\subsection{Regular Advertising on Facebook}

Any user with an active profile and Facebook page can become an advertiser. All they need to do is activate their ad account, select a targeting audience, fine-tune parameters such as bidding, and they can automatically send ads to their desired audience~\cite{tospolitical}. This means that everyone with a Facebook account can spread content about products, ideas, or even malicious information and fake news.

Facebook offers a multitude of audience selection options that can enable advertisers to target in a way which is considerably more fine-grained than traditional online advertising platforms like Google~\cite{google}. Apart from traditional targeting options, like \emph{age}, \emph{gender}, \emph{location}, and \emph{language}, advertisers can use - and combine in formulas - a variety of \emph{attributes} to target users. % which may be inferred by Facebook or be provided explicitly by those users. 
Advertisers can target users that have their birthday next month, or are interested in common subjects like \emph{Games} or \emph{Food}, but they can also target users interested in much more sensitive attributes such as \emph{Homosexuality}, or \emph{Fascism}. In fact, there exist more than 240,000 available attributes for advertisers to choose from~\cite{speicher-2018-targeted}, including at least 2092 potentially sensitive attributes~\cite{cabanas2018unveiling}. Additionally, advertisers can target users through \emph{custom audiences}~\cite{speicher-2018-targeted} by uploading to Facebook lists of users' Personally Identifiable Information (PII), such as phone numbers, emails, or names and physical addresses. Or, they can target \emph{lookalike audiences}, users that resemble some another desired user group according to Facebook~\cite{lookalike}.  These targeting options are naturally not only at the disposal of benign advertisers, but also malicious advertisers with ill intents. 


%Ad explanations look like as shown in Figure \ref{fig:ad_explanation}: 
%\begin{figure}[ht]
%\includegraphics[width=0.7\columnwidth]{figures/ad_explanation.png}
%\caption{Ad explanation sample.}
%\label{fig:ad_explanation}
%\end{figure}
%Every ad includes this button, and when users click on it, they get an explanation on why they are seeing the particular ad. Ad explanations typically have two parts: the first part presents one reason on why a user received an ad. Its wording is usually indicative of the type of attribute that it presents. 

%The second part lists potential attributes that might have been used by the advertiser in the targeting of an ad. It usually includes a limited set of information such as age, gender and location used as targeting options. 
%and also suggests that it is not sure that these attributes were used in the targeting. A typical example looks like ``There may be other reasons you're seeing this ad, including that The New York Times wants to reach people ages 18 and older who live in Germany. This is information based on your Facebook profile and where you've connected to the internet.'' 


\if 0
\paragraph{Ad preferences page}
The Ad preferences page is a customized page that provides users with information over the several attributes that influence the ads they consume, as well as it provides them with a certain level of control over them. First, users can view the interests that Facebook has inferred about them, such as whether they are interested in things like ``Video Games'', ``Pizza'', or even ``Homosexuality''. Interests are also accompanied by a description of how they were inferred. These descriptions can be statements like ``You have this preference because you clicked on an ad related to \emph{Interest}'', or ``You have this preference because you liked a page related to \emph{Interest}''. As it is shown in \cite{andreou2018investigating}, the overwhelming majority of these explanations is vague without providing a lot of details.
%
Additionally, Facebook provides users with information on behavioral and demographic information that the platform has inferred about them, like whether they are expats, or whether they are using Gmail, as well as information from their profile that can be used to target them such as their education level or their employer.
%
Moreover, the Ad preferences page includes information about advertisers that the user has interacted with. These can be (i) advertisers that have created a list with the contact info of a user, (ii) advertisers whose website or app the user has visited, (iii) advertisers whose ads the user has clicked and (iv) advertisers whose store the user has visited. 
%
Finally, users can remove specific interests, behaviors, demographics, profile data and advertisers that they don't wish to be used in their targeting. However, this doesn't affect the number of ads users are going to receive. Instead, it affects only the type of ads that will appear to them.
\fi 

%These targeting options are naturally not only at the disposal of benign advertisers, but also malicious advertisers with ill intents. In order to mediate concerns, 

%\vspace{2mm}
%\noindent \textbf{Advertising political content on Facebook:}
\subsection{Political Advertising on Facebook}

Regardless of Brazilian (or any other country) regulations, advertisers who want to send political ads on Facebook are subject to higher levels of scrutiny and the corresponding ads are subject to higher levels of transparency. Facebook defines an ad as political when~\cite{facebook_issue_content, facebook_political_content}:
\begin{trivlist}
\item \textit{(i) it is made by, on behalf of or about a current or former candidate for public office, a political party, a political action committee or advocates for the outcome of an election to public office; or}
\item  \textit{(ii) it relates to any election, referendum or ballot initiative, including "get out the vote" or election information campaigns; or (iii) it relates to any national legislative issue of public importance in any place where the ad is being run; or}
\item \textit{(iv) it is regulated as political advertising.}
\item \textit{(v) it is related to issues of public importance: abortion, budget, civil rights, crime, economy, education, energy, environment, foreign policy, government reform, guns, health, immigration, infrastructure, military, poverty, social security, taxes, and terrorism}
\end{trivlist}
Note that this is not the only definition for what is a political ad and scholars and regulators are currently debating about definitions~\cite{whatispoliticalfacebook}.

To sponsor political content on Facebook, advertisers need to first verify their accounts, declare that their ad is about political or social issues and put a disclaimer that mentions who paid for the ad.\footnote{\url{https://www.facebook.com/business/help/208949576550051?id=288762101909005}}


\if 0
\update{To help advertisers comply with the  2018 Brazilian Elections, the Facebook has changed its Term of Service with some new rules~\cite{tospolitical}}:  

%\oana{is this true?}
% Yes, this facebook link (in the reference) talk about this https://www.facebook.com/business/help/1256706951128601

\begin{trivlist}
\item ($i$) all advertisers that place political ads should be verified and identified by their Brazilian tax id (CPF or CNPJ); 
\item ($ii$) all political ads must be tagged as such before going live and, 
\item ($iii$) the money spent on advertisement must be declared to Brazilian authorities.   
\oana{is this something that facebook asks or is just brazilian legislation?}
% We dont known if in another countries  the electoral ad have to  be declared for authorities as Brazil does.
\end{trivlist}

Figure~\ref{fig:ad_anastasia} shows a snapshot of a legal official political ad made by a candidate during the election period. The information balloon ``Propaganda Eleitoral'' as well as the gray text just below the candidate's name inform that this is an official political ad and provide the identification of who paid for it.  
\fi 

%\vspace{2mm}
%\noindent \textbf{The Facebook Ad Library:}
\subsection{The Facebook Ad Library}
The ads declared by  advertisers as containing political content are part of the historical Facebook Ad Library. 
While Facebook provides functionalities for advertisers to include disclosure information about their political ads, we do not know whether Facebook has any kind of enforcement mechanisms for detecting political ads that do not have the appropriate disclosure in Brazil.

%\oana{@Fabricio, is this right?}



\if 0
\begin{itemize}
    \item Is made by, on behalf of or about a current or former candidate for public office, a political party, a political action committee or advocates for the outcome of an election to public office; or
    \item Relates to any election, referendum or ballot initiative, including "get out the vote" or election information campaigns; or
    \item Relates to any national legislative issue of public importance in any place where the ad is being run; or
    Is regulated as political advertising.
    \item Issues of public importance: abortion, budget, civil rights, crime, economy, education, energy, environment, foreign policy, government reform, guns, health, immigration, infrastructure, military, poverty, social security, taxes, and terrorism.
\end{itemize}
\fi 



==> WWW-CONF 2/3-dataset.tex <==
\section{System for Monitoring Ads}
\label{sec:dataset}

This section describes our tool and the datasets we collected for this study.


\subsection{Tool Design}

Our tool is a browser extension (for Chrome and Firefox) that collects the ads that appear in the Facebook feed of the volunteers who install it. 
We forked \adanalystbr from \adanalyst\footnote{\url{https://adanalyst.mpi-sws.org/}}, and we added support for collecting and analyzing ads in the Portuguese language as well as an interface in Portuguese where users can browse the ads we collect. 

%\adanalystbr was adopted for Brazilian audiences. %a transparency tool that collects Facebook ads from users, as well as information from Facebook's transparency mechanisms, and provides aggregate statistics to users to help them make more sense of the ads they receive in Facebook. 

%In this work, we use Facebook ads collected by \adanalystbr\footnote{Name modified due to double-blind process.}, a browser plugin we developed to collect the ads that appear in the Facebook feed of volunteers who install it.  We refer the reader to Section \ref{subsec:deployment} for more details on the ad collection methodology.

To capture the ads that users receive on Facebook, we scrape the Facebook's HTML and we look  for the tag \emph{``Sponsored''} (\emph{``Patrocinado''} in Portuguese). This tag is used by Facebook to help users distinguish sponsored content from the rest. %\update{Recall that Brazilian law stipulates strict rules for sponsored content during the election period.} 
The captured frame contains the media content of the ad (either a video, an image, or a collection of images), the text of the ad, and a link to the advertiser's page. Our browser extension does not collect ads that appear when a user is watching a video on Facebook.

Facebook provides explanations to users on why they have received a specific ad. To obtain such explanations, users need to click on the ``Why am I seeing this?'' button that is in the upper right corner of every ad.  These explanations provide some information regarding the parameters set by the advertisers, but not all~\cite{andreou2018investigating}. We also instrument the browser extension to collect these explanations. 

\paragraph{Ethical considerations:}
We only collect information about the ads and clearly state what we collect to the volunteers who install the extension and accept our terms. We do not collect any information about friends list, likes, photos, videos or regular timeline posts.
Furthermore, the code of our extension is open source and it is publicly available~\footref{dataset}.

\subsection{Dissemination and Deployment}

The initial users who installed our browser extension were friends and family. Later, our browser extension was widely adopted after our project was cited by popular national and international news media outlets such as BBC, El País, Finantial Times, and Folha de São Paulo~\footnote{\url{http://www.eleicoes-sem-fake.dcc.ufmg.br/?section=midia}}. 
Additionally, to disseminate the tool, we  wrote and published opinion articles to  disclose ways to exploit online systems to influence elections and what we can do about them~\cite{fabriciofolha,nyt2018benevenuto}. These risks were then exposed by our team in the Brazilian senate and in multiple national TV shows\footnote{\url{https://www.youtube.com/watch?v=eGScrdi5hhU&t=3450s}.}.

%We used \adanalystbr to monitor ads from March 14, 2018 to October 28, 2018. This period covers the electoral period, including the two voting rounds. Overall, more than 2,000 users volunteered to install our browser extension and share the ads they received while navigating on Facebook with our project. We noted, however, that many users only installed the browser extension but do not used. Nevertheless, a total of $715$ users actively used our tool in this period. 

%The Brazilian election period was divided into two rounds: the first round started on August 16, 2018 and ended on October 7 and, the second round started on October 8, 2018 and ended on October 28. 

%As political ads only are considered electoral ads and require to follow special rules in August 16, 2018, we collected ads both from the period before the electoral period and also along the entire electoral period, covering both voting rounds. 



\subsection{Data Collection}

\begin{figure}[t]
\includegraphics[width=0.6\columnwidth]{plots/timeline_active_users_per_day}
\caption{Number of daily active users.}
\label{fig:user_by_day}
\end{figure}

We used \adanalystbr to monitor ads from March 14, 2018 to October 28, 2018. This period covers the electoral period, including the two voting rounds. Overall, more than 2,000 users volunteered to install our browser extension and share the ads they received while navigating on Facebook with our project. We noted, however, that many users only installed the browser extension but do not used it. Nevertheless, a total of 715 users actively used our tool in this period. 


Figure~\ref{fig:user_by_day} shows the number of active users per day. We consider a user as active in a day if they received at least one Facebook ad. The number of daily users increased rapidly when several news-media outlets published articles about our system and stayed relatively stable afterward. The sudden decrease of active users in mid-June can be attributed to a change Facebook makes in the way it tags ads, resulting in the loss of ads for some days. We also notice that user activity on weekends decreases, which might indicate that some users have installed our plugin in their computer at work.
%\update{Because the tag of official political ads is different, besides ``Patrocinado'', the disclaimer also contains the tag ``Propaganda Eleitoral'', our extension did not collect these ads in the months before the election. Hence, the dataset collected with our browser extension does not contain official political ads.}  



%\update{Due to a change in Facebook's way of displaying ads, some of the official political ads that use a tag ``Propaganda Electoral'' were not collected by our extension. Therefor we cannot guarantee that we collect ads from Facebook Ad Library.}  \oana{Thanos did a check and we do not collect any official political ad} \oana{so this paragraph needs to change}


%\oana{how did we inferred that they are from brazil?}

%\begin{table}[h]
%\caption{Geographical distribution of users in our dataset.} 
%\label{tab:dataset}
%%\vspace{-2mm}
%\small{
%\begin{center}
%\begin{tabular}{c|c|c|c}
%%\begin{tabularx}{\columnwidth}{l|p{0.07\columnwidth}p{0.20\columnwidth}p{0.40\columnwidth}}%s\cline{2-3}
%% & \multicolumn{3}{c}{\datasetBrazil} \\
%{\bf Location} & {\bf Users} & {\bf Unique Ads} &  {\bf Unique Advertisers}
%%South America  & 683 & 224K & 36K  \\
%%Europe  & 9 & 9K & 3K  \\
%%North America  & 8 & 6K & 2K  \\
%%Africa  & 1 & 336 & 136  \\
%
%\\ \hline
%Brazil  & 682 & 224K & 36K  \\
%United States  & 5 & 4K & 2K  \\
%Canada  & 3 & 2K & 831  \\
%Other & 11 & 9K & 878\\
%Unknown  & 14 & 514 & 291  
%\\ \hline
%Total & 715 & 239K & 40K  \\
%\end{tabular}
%\end{center}
%}
%\label{tab:geographical-distribution-continents-dataset}
%%\vspace{-7mm}
%\end{table}%

%\textbf{Geography}: In the Table \ref{tab:geographical-distribution-continents-dataset} we show the geographical distribution of users in our dataset. %We use the same method proposed by Andreou \textit{et al.}~\cite{Andreou19a}.

Out of the 715 users, 682 are from Brazil. We inferred this targeting information by parsing the data from the "\emph{Why am I seeing this?}" explanations that were collected by our extension~\cite{andreou2018investigating}. 
We collected in total \textbf{239k unique ads} sent by \textbf{40k advertisers}. Each ad is identified by an unique \emph{id} provided by Facebook. %\oana{what is the difference between ads and unique ads? in the rest of the paper do we consider only unique ads? are the 1000 ads we detect as political unique ads?} 
%The average number of unique ads per day can range from $1.5$ to $99.5$ for each user, with a median of $10$ per day.
Out of the 239k unique ads, 166k were sent during the pre-electoral period (March 2018 to August 15, 2018) and 74k were sent during the electoral period (August 16, 2018 to October 28, 2018). For each ad we have information about the advertiser, the text of the ad, the text in the political ad disclaimer, the image (when available) and the landing URL. We refer to this dataset as the \emph{\adanalystbr dataset}.

 Official political ads are different than regular ads. Besides the ``Sponsored'' tag, the disclaimer also contains the tag ``Electoral Propaganda''. Because of that, our extension did not collect these ads, i.e., the dataset collected with our browser extension does not contain any official political ad.
 
 
\if 0
\paragraph{Image Features}
\update{We gathered features from ad containing images using Google Cloud Vision API~\cite{google_cloud_api}. It consists of a pre-trained machine learning models able to label a number of elements in an image, associating category labels to the image according to the elements identified in it. Additionally, it identifies printed and handwritten text. We have particularly explored this feature as an attempt to identify text words in an image that is associated to a political propaganda. We extracted features from $20,851$ ad images, these images belong to our $10,000$ labeled ads. Our main goal using this api is extracting text from these ad images.}
\fi


%through REST and RPC APIs. Assign labels to images and quickly classify them into millions of predefined categories. Detect objects and faces, read printed and handwritten text, and build valuable metadata into your image catalog \cite{google_cloud_api}. We extracted features from $20,851$ ad images, these images belong to our $10,000$ labeled ads. Our main goal using this api is extracting text from these ad images.}


%\subsection{\Fbdata dataset}
\subsection{Facebook Ad Library Dataset}

Facebook provides an Ad Library that includes all ads that were declared as containing political content by the advertisers~\footnote{\url{https://www.facebook.com/politicalcontentads}}. The Ad Library offers a search engine where given a keyword, the engine returns matching advertisers and their ads. Facebook lists the top 30 results for the query and provides a token for the next page.  We implemented a crawler to perform automatic searches and scrape the results provided this application. 
In August 2018, the search engine allowed to query empty strings and was returning a long list of ads sorted by the publish time. We collected all the returned results until the last page. Unfortunately, the Facebook Ad Library changed a lot during the past 2 years, which might make this collection method not possible anymore~\footnote{The task of building and maintaining this crawler is not straightforward.  Facebook constantly updates the URL parameters of search queries and implements countermeasures to detect and block crawlers.}. 

We tried to collect close to all ads declared as political. To do that, we repeated the task of querying for an empty string periodically during the period of Aug 2018 to December 2019, a total of 11 complete crawls.  Each additional crawl increased our dataset by an average of 2.63\%. %\oana{did the dataset increased by 2.6\% with the 11 crawls combined, or for each crawl it increaded by 2.6\%?}
Additionally, to measure how many ads we missed, we performed a hundred searches with distinct random words selected from a Wikipedia dataset~\cite{wikipedia_dataset}. This experiment revealed that our dataset increased, in total, by 2.59\%, or by an average of .0259\% for each search.
While we believe we are close to have the entire dataset of political ads, there is not a systematic way to assess the amount we of ads we did not gathered. As also observed by others, the Facebook Ad Library is unstable and there are ads that appear and ads that disappear each day which makes it impossible to know for sure how many ads we miss~\cite{mozillaadlibraryreport}.

For each ad, Facebook returns the advertiser's name, the advertiser's Brazilian tax id, the ad text, the ad media (video or images), how much money was spent on the ad and information about the age, the gender and the location of the users reached.  We filter out ads that did not reach people in Brazil and are not marked as being about political, election and social issues.\footnote{The new version of the Ad Library also returns active campaigns of advertisers that can include ads that are not political. We exclude these ads from the dataset as well.} %Our main focus is gathering ads that ran during electoral period and detect possible misuse of Facebook Ad Platform. 
Our curated dataset contains \textbf{100,778 unique ads} from \textbf{5,292 advertisers} during the electoral period and all ads gathered are specific to Brazil.
%\oana{do we also keep only the ads during the electoral period? if yes we should mention this in the previous paragraph}
We refer to this dataset as the \emph{\Fbdata dataset}.
%\oana{how is the filtering by date impacting the fact that 1000 political  are not in the Ad Library? }
% \marcio{all analysis focused in electoral period, these 1000 ads are included in these period}

%Our method was to simply search for empty queries 
%For this task, we make empty queries and we search for all political ads available at the time. Facebook lists the top 30 results for the query and provides a token for the next page. It doesn't show how many ads the query returned in total, but we make the crawler go to the last page. 



 

 
 
 

 

 

% In addition to the \adanalystbr dataset, we also collected another dataset from official political ads provided by Facebook Since October 6, 2017 by law, all advertisers who created political ads have to tag their ads as ``political'' and provide their Brazil tax id called CPF or CNPJ~\cite{cod_rights_2018}. 
 
% Users can then use Facebook's search engine for political ads where they can search for advertisers who sponsored any political content. 
 
 

 


%\thanos{@marcio: if we filter only ads that are in Brazil, when we detect the political ads that Facebook has not added by intersecting them with our dataset, are we sure that they are not just from some other country}

%\thanos{@marcio: if we filter only ads that are in Brazil, when we detect the political ads that Facebook has not added by intersecting them with our dataset, are we sure that they are not just from some other country}

%At August 2018, Facebook did not provide an official API. So, we had to build a crawler, which needs to be updated constantly due to the fact that Facebook constantly updates URL parameters of this search and also countermeasures to detect crawlers, then our crawler worked slowly preventing blocks. We run this task periodically searching for new ads. Additionaly, we make a experiment performing searches with $100$ random words selected from wikipedia dataset\cite{wikipedia_dataset} in order to measure how many ads we missed. Then, this experiment revealed that our dataset increased only $2.6\%$ the number of ads.
%
%
%


\if 0
\paragraph{Twitter dataset}
Finally, we also used a dataset of $2K$ political tweets from $659$ public Brazilian deputies~\cite{oliveira2018} to train our classifiers. In this dataset, Oliveira et al.~\cite{oliveira2018} labeled $1,000$ tweets as \textit{political} and $1,000$ as \textit{non-political}, evenly distributed across deputies and across time, to make the classifier able to accurately classify political tweets independently of the deputy who posted it and of the time it was posted. They also validated the dataset among three independent researchers and obtained a majority vote Cohen's Kappa coefficient~\cite{Landis1977} equals to 0.73 and 86\% of agreement.
\fi 


==> WWW-CONF 2/4-classifier.tex <==
\section{Detecting political ads} \label{sec:methodology}

There is no consensus on what is a political ad. Different platforms have different definitions for what they consider as political ads~\cite{twitter_ban_political_ad,google_pol_ads}, while at the same time political scholars and regulators are debating about what would be a good definition~\cite{pda}. 

Our goal in this work is not to provide the best definition for a political ad, but to operationalize one that is able to identify ads that are similar to self-declared political ads.  More specifically, our approach consists on  investigating to which extent we can build machine-learning algorithms that are able to accurately identify similar ads from those available in the Facebook political Ad Library. 

%political according to \emph{some reasonable definition}, even if the definition is not perfect. 

%Thus, our approach consists of identifying a machine learning model able to correctly distinguish between a self-declared political ad from the Facebook ad archive from a non-political ad. 

%focus here is to design a data-driven approach to  operationalize the concept of `political ad', i.e., to provide a data-driven definition for political ad that allows us to automatically detect it. 

In practice, our approach has three key steps. First, we need to create a gold standard collection of ads used to test our method. Then, we select a supervised classifier that receives as input an ad and outputs if it is political , i.e., of the same nature as the ones registered as such on Facebook, or non-political. Finally, we evaluate this classifier over different sets of testing data.



%\subsection{What is a political ad?}

%In this paper our focus is on investigating to which extent we can build machine-learning algorithms that are able to detect ads that are political according to \emph{some reasonable definition}, even if the definition is not perfect. 
%We consider as political ads the ads declared on Facebook as \emph{Political and Issue ads} as well as ads that correspond to the definition proposed by Oliveira \textit{et al.}~\cite{oliveira2018}:
%\newtheorem{p_def}{Definition}
%\begin{p_def}
%\label{def1}
%A \textbf{political advertisement} in Facebook is a sponsored message posted on a Facebook page whose content expresses subjects related to state, politics, governance, and justice. Specifically, such messages may cover one or more of the following topics: political campaign; human rights; political activism; political news; federal programs projects and laws; politician public agenda; judicial decisions; public expenditures and crimes against public administration.
%\end{p_def}

%Our thinking is that there should be a set of ads that irrespective of the definition, people agree that they are political. The focus of this section is to investigate the feasibility of detecting political ads using machine learning-based methods, hence, we focus on detecting at least the ads that are clearly political. % and we leave discussions around detecting more controversial ads for future work. 
%\oana{is ok this argument argument?}

% \oana{the biggest difference I see is the inclusion of ads from news media}

%In Section 5, we provide Definition~\ref{def1} as part of the instructions to volunteers in order to label ads as political and non-political, which we used to evaluate our system. 


% Pressured by academics, including our team\footnote{Opinion article omitted due to the double-blind process} and journalists, Facebook agreed with the Brazilian authorities to adopt new rules for Brazilian Elections, which regulate advertisers for placing political ads along the election period:
%
%\begin{itemize}
%\item All advertisers that place political ads should be verified and identified by their Brazilian tax id (CPF or CNPJ);
%\item All political ads must be tagged as such before going live;
%\item Money spent with advertisement must be declared to Brazilian authorities;
%\end{itemize}



%In Section 6, we gathered the official dataset of political ads and contrast those ads with the ads we gathered from volunteers who installed our browser add-on. 


\subsection{Gold standard collection}\label{sec:labeling-ads}

To train and test our machine learning models we need a labeled set of political and non-political ads. Next, we describe our assumptions and how we create a set of political and non-political ads. \\

\noindent
\textbf{Political ads}: As political ads, we choose a uniformly distributed random sample of $10,000$ ads from the \Fbdata dataset.
As these ads were made by political candidates or political parties as part of their official political campaigns, they are good representative instances of political ads for training our machine learning-based methods. 
Our rationale is that, independent of the definition of a political ad, our data-driven approach  might be able to properly recognize an ad that is similar to those self-declared political ads made by real political agents. \\

\noindent
\textbf{Non-political ads}:
There are no available existing labeled datasets for non-political ads. 
Thus, we need to label such ads ourselves. We selected a uniformly distributed random sample of $10,000$ ads from the \adanalystbr dataset. Although most of the ads in this dataset are not about politics, there are a few political ads among them. So, we asked three independent volunteers\footnote{The volunteers were students in our lab.}  to label the ads as political or non-political. We instructed the volunteers to consider as political ads the ads declared on Facebook as \emph{Political and Issue ads}, as well as ads that correspond to the definition proposed by Oliveira \textit{et al.}~\cite{oliveira2018}:
\newtheorem{p_def}{Definition}
\begin{p_def}
\label{def1}
A \textbf{political advertisement} in Facebook is a sponsored message posted on a Facebook page whose content expresses subjects related to state, politics, governance, and justice. Specifically, such messages may cover one or more of the following topics: political campaign; human rights; political activism; political news; federal programs projects and laws; politician public agenda; judicial decisions; public expenditures and crimes against public administration.
\end{p_def}



%Our thinking is that there should be a set of ads that irrespective of the definition, people agree that they are political. The focus of this section is to investigate the feasibility of detecting political ads using machine learning-based methods, hence, we focus on detecting at least the ads that are clearly political.

We evaluated the inter-rater reliability among the independent volunteers using the agreement percentage and the Cohen's Kappa coefficient ($\kappa$)~\cite{Oren2011,Landis1977,Savage2015}. This coefficient measures the agreement between two volunteers who each classify a predefined number of ads as one of the two mutually exclusive categories: \emph{political} or \emph{non-political}. The agreement among the three volunteers is consistently very high, 99.7\% for volunteers 1 and 2, with $\kappa = 0.93$, and 99.5\% for volunteers 1 and 3, with $\kappa = 0.88$. For volunteers 2 and 3 the agreement is 99.5\%, with $\kappa = 0.89$. According to Landis and Koch~\cite{Landis1977}, these Kappa scores fall into the range of scores referred to as ``Almost Perfect'' agreement, which is a satisfactory result that validates our \textit{gold standard collection}.
The labeled data contains $233$ political ads and $9,767$ non-political ads. We added the $233$ political ads as part of our political ads dataset. 
Our final \gs collection is a nearly balanced dataset containing \textbf{10,233} political ads and \textbf{9,767} non-political ads.\footnote{This dataset is publicly available to download at \url{https://lig-membres.imag.fr/gogao/political_ads.html.}} 


%The 233 political ads are not enough to train and test classifiers reliably. To increase the number of labeled political ads we randomly picked 10k ads from the \Fbdata dataset.  As these ads are made by politicians and political parties as part of their official political campaigns, we found it unnecessary to relabel those ads.  


%As a contribution to the scientific community, we plan to make this dataset available in due time. 

%\begin{table}[ht]
%\centering
%\caption{Cohen's Kappa and Agreement percentage among researchers over \textit{labeled training set} containing $10,000$ Facebook ADs}
%
%\label{tab:labeled}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{lccc}
%\hline
% & & \textbf{Researchers} \\
%\hline
%	&	\textbf{1 and 2}	&	\textbf{1 and 3} & \textbf{ 2 and 3} \\
%\hline
%Kappa coefficient $\kappa$	&	0.93	&	0.88	&   0.89 \\ 
%Agreement \%			&	99.7\%	&	99.5\%  &   99.5\% \\
%\hline
%\end{tabular}
%}
%\end{table}




%To appropriately train and test our model, we opted to have at our disposal a large set of political ads and non-political ads. The \textit{\update{Facebook Ad Library}} contains only political ads. 
%As we described in Section 3, we have crawled $100,778$ political ads related to the 2018 Brazilian elections. 


%On the other hand, we have at our disposal a dataset of $239K$ unique ads collected from \adanalystbr that might contain both political and non-political ads. 







 %\thanos{@marcio,@all: so the volunteers find 233 political ads in a random 10K sample, and our algorithm detects 1,128 political in 240K ads?}
%\marcio{we are interested in election period (August 16, 2018 - October 28, 2018)}
%\thanos{@all: Also, I see that  in section five that the 233 ads are included in the 1,128? @all: should we maybe remove these 233 from the number, they are 20\% of our reported new ads and they are not really detected by our model, we just trained the model using them.}
%yes, i will update the venn diagram
%\thanos{@marcio:Is any of the ads we take in the sample from adanalyst also part of the sample that we take from the  political ad archive?}
%\marcio{@thanos, We have to investigate, but manually it is hard task}

\subsection{Supervised learning algorithms}

We evaluate five classifying techniques to distinguish between political and non-political ads: Logistic Regression, Random Forest, Support Vector Machine with RBF kernel, and Gradient Boosting using Grid Search for selecting best hyperparameters during the train and Word Embedding for feature extraction, and Naive Bayes using Hashing Vectorizer for feature extraction.
%\oana{@marcio did you set up any specific parameters for this classifiers?} \oana{@Marcio, did you used word embeding with this classifiers?} 
% we use grid search, 


We also implemented a Convolution Neural Network (CNN) architecture recently proposed for a similar task: identifying political tweets posted by politicians~\cite{oliveira2018}. Figure~\ref{fig:cnn_model} presents an overview of our implementation.  We represent each word of a Facebook ad as a dense vector retrieved from Word2Vec C-BoW with 300 dimensions, pre-trained over a large Portuguese data set, which is able to produce an embedding matrix for a vocabulary of 1.3 trillion terms~\cite{Mikolov2013,Hartmann2017}. Thus, the input layer is a matrix $n \times 300$, where $n$ is the number of words in a particular ad and $300$ is the vector representation of each word of this message. Subsequently, there is a 25\% rate dropout regularization layer connected to a convolutional layer with $120$ different filters and sizes (3,4,5), activated by a ReLU function. Then, the output of the previous layer is connected to a global max-polling layer, whose output is in turn, fully connected to a ReLU activation and to another 25\% rate dropout layer. Finally, the last dense layer is a single neuron with a sigmoid activation function that outputs $1$ if the message is \textit{political}, and $0$ if \textit{non-political}. We optimized the neural network by means of cross entropy loss function using the RMSProp optimization algorithm~\cite{Duchi2011}.
 

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\linewidth]{figures/cnn_model_noborders.png}
\caption{Convolutional Neural Network architecture for political ads classification. 
%\oana{can you remove the borders of this image? the image is very ugly} FIXED
}
\label{fig:cnn_model}
\end{figure*}

 
\subsection{Evaluation}

\if 0
 \update{Our \textit{gold standard collection}, contains $233$ political and $9,767$ non-political advertisements manually labeled. In addition to this collection, we consider the another dataset described in Section~\ref{sec:dataset} for gathering textual features used to train and test our models:  the \textit{Official Political Facebook ads}, whose we randomly selected $10,000$ official political ads. Then, our train and test dataset has $20,000$ ads splitted in 10-\emph{folds}, $90\%$ for train and $10\%$ for test. In order to evaluate our choice of the classifier, we also run the results for four classic supervised baselines: Logistic Regression, Gradient Boosting, and Naive Bayes.}
 \fi 
 
We use 10-fold cross validation to train and test the six classifiers. We partition the \gs dataset in ten random sub-samples, out of which nine are used as training data, and the remaining one is used for testing the classifier.  The results reported are averages of the 10 runs along with their 90\%-confidence intervals. 
 
\if 0 
 \update{In order to add extra textual feature to Lebaled Ads, we extracted texts from the all image in Labeled Ads, then we added to train. Our main goal adding these extra feature is investigated whether the model performance would be better than previous analysis without ad image features. In total, $7,598$ out of $10,000$ labeled ads had text. }
\fi 

\if 0
\begin{table}[htb]
\small
  \caption{Text features for training and validation}
  \label{tab:features}
  \begin{tabular}{clccc}
    \toprule
    
    \textbf{Abbrv} & \textbf{Text feature} & \textbf{pol.} & \textbf{non-pol.} & \textbf{Total}\\
	
    \toprule
    $S1$ & Labeled Tweets  & $1,000$ & $1,000$ & $2,000$\\
    $S2$ & Labeled Facebook Ads & 233 & 9,767 & 10,000\\
    $S3$ & Official Political Facebook Ads\footnote{https://www.facebook.com/politicalcontentads} & \update{26,059} & 0 & \update{26,059}\\
  \bottomrule
\end{tabular}
\end{table}
\fi

To evaluate the classifiers we considered three classic metrics: accuracy, Macro-F1, and the area under the ROC curve (AUC). Accuracy considers equally important the correct classification of each ad, independently of the class, and basically measures the capability of the method to predict the correct output. As the \gs dataset is nearly balanced, the results for accuracy are meaningful. The resulting AUC is the probability that a model will rank a randomly chosen political ad higher (e.g. more political) than a randomly chosen ad. The AUC is especially relevant for political ad detection since the decision threshold can be used to control the trade-off between true and false positive rates. Finally, Macro-F1 values are computed by first calculating F1 values (a metric that captures both precision and recall for a 0.5 threshold) for each class in isolation, then averaging over all classes. This way, Macro-F1 considers equally important the effectiveness in each class, independently of the relative size of the class. Besides that, the Macro-F1 score is the harmonic mean of the precision and recall.%, where an F1 score reaches its best value at 1 (perfect precision and recall)\cite{macrof1sasaki}. %and   \oana{if we have a near balanced dataset is it important to compute the macro-F1 score?}


Table~\ref{tab:results_experiments} presents the accuracy, AUC and Macro-F1 score for the six classifiers we consider. The accuracy of CNN, SVM, Logistic Regression and Naive Bayes is 94\% in a nearly balanced dataset for detecting both political and non-political ads. 

%\begin{figure}[!ht!]

%\includegraphics[width=1.0\columnwidth]{plots/roc_curve.png}
%\caption{ROC curves for our classifiers} }
%\label{fig:roc_result}
%\end{figure}



While our classifiers achieve an impressive accuracy in a nearly balanced dataset, in the real-world the number of non-political ads is much higher than the number of political ads. Hence, it is important to study the ROC curves of classifiers and what true positive rates (detection of true political ads) they achieve for small false positive rates (false detection of non-political ads as political ads).  %Figure~\ref{fig:roc_result} shows the corresponding ROC curves for all classifiers, we calculated the average of ROC Curves over the 10 folds. In addition, 
Table~\ref{tab:results_tpr} shows the true positive rate for a false positive rate of 1\% and 3\%. We observe that CNN and Naive Bayes classifiers are the most accurate with true positive rates of 78\% and 85\% for a 1\% false positive rate.
%\oana{@Marcio please do this table, or send the data to thanos and he can do this table}

%\update{Even the CNN presented TPR under Naive Bayes, deep learning models were built to accepted large datasets each new elections, local or federal elections. Chen~\cite{chen_deep_learning} discussed in your work several CNN advantage over Machine Learning techniques. For instance, the CNN can be scaled to huge amount of data and always growing the accuracy.} \oana{i did not get this point}

%\oana{add interpretation of resutls after you make the table}

%Table~\ref{tab:result_table} shows further provide details for precision, recall and F1 for each class. We can note that CNN has a better precision in detecting political ads ($0.97$) in comparison with SVM, logistic regression, and Naive Bayes. Because of that, we choose to deploy the CNN algorithm in our system.
%Finally, Figure~\ref{fig:roc_result} presents the ROC curve for all classifiers.  Inspecting the ROC curve for CNN (Figure~\ref{fig:roc_result} (a)), we can  
%observe that it is possible to choose a threshold in which the classifier is able to correctly classify nearly all of political ads (true positive rate $\approx$ 1), while misclassifying only $25.25\%$ of the non-political ads (false positive rate $\approx$ $0.25$). This can be useful, especially in a scenario in which one wants to identify ads that are worth investigating. Conversely, in the next section, we explore this kind of parameter to deploy a system able to properly identify part of the political ads, but with a low rate of false positives, that are non-political ads classified as political. 

%A variation of F1, namely, Macro-F1, is usually reported to evaluate classification effectiveness on skewed datasets.  


%\thanos{Do we really care about Macro F-1? We do not really use it anywhere. Why not remove it?}
%\marcio{Macro-F1 it is important metric to compare classifiers in classification problem. }

%In the training process we used $10$\emph{-fold} \emph{cross-validation}. 
%For each test fold $i$, we trained the model with the rest, until all folds have been used as test fold. Then, we calculate the mean and confidence interval for each class metrics (\emph{precision}, \emph{recall}, \emph{f1}), also \emph{Macro-F1}, \emph{AUC - Area Under the Roc Curve}  and \emph{accuracy}. 

%We can see from Table~\ref{tab:results_experiments} that four classifiers are tied as best option for the task in terms of accuracy and AUC. More important, the performance of these classifiers is quite impressive (94\% of accuracy in a near balanced dataset), correctly predicting almost all political ads and misclassifying only a small fraction of the non-political ones.  


%\begin{table}[t]
%\centering
%\tiny
%\caption{Accuracy of different classifiers}
%\label{tab:results_experiments}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{lcc}
%\hline
%	\textbf{Classifier} &	\textbf{Accuracy}	&	\textbf{AUC}  \\
%\hline
%\textbf{CNN} 	        & \boldmath$0.94 (\pm 0.01)$	& \boldmath$0.98 (\pm 0.01)$ \\ 
%\textbf{SVM} 			& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.98 (\pm 0.01)$ \\
%\textbf{L. Regression} 	& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.98 (\pm 0.01)$ \\
%R. Forest 		& $0.92 (\pm 0.01)$	& $0.97 (\pm 0.01)$ \\
%\textbf{N. Bayes} 		& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.99 (\pm 0.01)$ \\
%G. Boosting 	& $0.92 (\pm 0.01)$	& $0.97 (\pm 0.02)$ \\
%
%\hline
%\end{tabular}
%}
%\end{table}





\begin{table}[t]
\centering
%\begin{small}
\caption{Accuracy of different classifiers.}
\label{tab:results_experiments}
%\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
	\textbf{Classifier} &	\textbf{Accuracy}	&\textbf{AUC} & \textbf{Macro-F1}  \\
\hline
\textbf{CNN} 	        & \boldmath$0.94 (\pm 0.01)$	& \boldmath$0.98 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\ 
\textbf{SVM} 			& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.98 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
\textbf{L. Regression} 	& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.98 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
R. Forest 		& $0.92 (\pm 0.01)$	& $0.97 (\pm 0.01)$ & $0.92 (\pm 0.01)$\\
\textbf{N. Bayes} 		& \boldmath$0.94 (\pm 0.01)$  & \boldmath$0.99 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
G. Boosting 	& $0.92 (\pm 0.01)$	& $0.97 (\pm 0.02)$ & $0.92 (\pm 0.01)$ \\

\hline
\end{tabular}
%}
%\end{small}
\end{table}



\begin{table}[t]
\centering
%\begin{small}
\caption{True Positive Rate (TPR) for 1.0\% and 3.0\% False Positive Rate (FPR).}
\label{tab:results_tpr}
%\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\hline
	\textbf{Classifier} &	\textbf{FPR = $1\%$}	&\textbf{FPR $3\%$}  \\
\hline
\textbf{CNN} 	        & \boldmath$78\%$	& \boldmath$90\%$ \\ 
SVM 			& $57\%$  & $85\%$ \\
L. Regression 	& $58\%$  & $85\%$  \\
R. Forest 		& $62\%$	& $83\%$ \\
\textbf{N. Bayes} 		& \boldmath$85\%$  & \boldmath$95\%$ \\
G. Boosting 	& $57\%$	& $79\%$ \\

\hline
\end{tabular}
%}
%\end{small}
\end{table}



%\begin{table*}[t]
%  
%  \centering
%  \caption{Precision, Recall and F1 results. }
%  
%  %\thanos{We report the results based on one threshold for each model, right? Do we chose the threshold with the highest precision and then also calculate the Recall and F1?}
%  %marcio{this metrics are all calculated using the 0.5 threshold}
%  
%  \label{tab:result_table}
%    \begin{tabular}{|r|c|c|c|c|c|c|c|c}
%    	
%    \hline
%     \multicolumn{1}{|c|}{\multirow{2}[2]{*}{\textbf{Classifier}}} &  \multicolumn{3}{c|}{\textbf{Political}} & \multicolumn{3}{c|}{\textbf{Non Political}}  \\
%    
%                 & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \\
%
%\multicolumn{1}{|l|}{\textbf{CNN}} &  \boldmath$0.97 (\pm 0.01)$ & \boldmath$0.91 (\pm 0.03)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.91 (\pm 0.03)$ & \boldmath$0.97 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$  \\
%
%\multicolumn{1}{|l|}{\textbf{SVM}} &  \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.93 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$  \\
%\multicolumn{1}{|l|}{\textbf{L. Regression}}  & \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$  \\
%
%  \multicolumn{1}{|l|}{R. Forest} &  $0.95 (\pm 0.01)$ & $0.89 (\pm 0.01)$ & $0.92 (\pm 0.01)$ & $0.89 (\pm 0.01)$ & $0.95 (\pm 0.01)$ & $0.92 (\pm 0.01)$  \\
%  
%  \multicolumn{1}{|l|}{\textbf{N. Bayes}}  & \boldmath$0.91 (\pm 0.02)$ & \boldmath$0.99 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.98 (\pm 0.01)$ & \boldmath$0.90 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$ \\
%  
%  \multicolumn{1}{|l|}{G. Boosting}  & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.01)$  \\
% 
% \hline
%    \end{tabular}%
%  \label{tab:text_and_images}%
%  
%  
%\end{table*}%



%Also, we evaluate the classification performance of the each learning method considering each combination of textual features as input: $S1$, $S2$, $S3$, $S1 + S2$, $S1 + S3$, $S2 + S3$, $S1 + S2 + S3$. Our goal is to assess the discriminating power of adding each set of textual features and understand if adding features from tweets, for example, would add noise or help in differentiate political ads from the non-political ones.

%In Table~\ref{tab:tabelao2}, we show the results for all configurations of \textbf{input} and \textbf{method}. We highlight in bold all the configurations that achieved the statistically highest Macro-F1 scores. First, observe that using all datasets as input have not achieved the best results. In particular, adding $S3$ to the training phase harmed the performance of every classifier in comparison with using only $S1$ and $S2$. Recall that $S3$ contains only official Facebook political ads, and the performance of the classifier degraded probably because the characteristics of such ads are very different from the ones our system is expected to see in production ($S2$).

%Thus, considering all the possible combinations among $S1$, $S2$ and $S3$, as an effort to identify the best approach for our system, we observe that configurations using \update{$S1$ and $S2$}, yielded the best Macro-F1 scores. In particular, the CNN classifier with \update{$S1$ and $S2$} with text from $S2$ images is the one that achieved the best average result, with Macro-F1 \update{0.76} \update{($\pm0.06$) as shown on Table \ref{tab:text_and_images}. Adding text from $S2$ images on train improved our CNN model in $3\%$}. In fact, the CNN classifier was regularly the best method considering different sets of inputs. Also, note the increase in the Precision (\textbf{P}) scores for the political ads when $S2$ is added in the training phase of the model. This happened because $S1$ contains a set of political and non-political tweets posted by congressmen, which are helping the classifier to identify those political ads that are more subtle than traditional ``vote for Smith'' types of ads.


% \begingroup
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.0} % Default value: 1


% \endgroup
% \twocolumn

%Given these results, we have deployed three experimental versions of the system, each one deploying one of the models statistically tied as the best option. Three researchers individually evaluated these versions of the systems and unanimously preferred the model trained with Thus, we deployed the model trained with \update{$S1+S2$ and text extracted from $S2$ images} in our system.






%\begin{table*}[t]
%  
%  \centering
%  \caption{Precision, Recall and F1 results. }
%  
%  %\thanos{We report the results based on one threshold for each model, right? Do we chose the threshold with the highest precision and then also calculate the Recall and F1?}
%  %marcio{this metrics are all calculated using the 0.5 threshold}
  
%  \label{tab:result_table}
%    \begin{tabular}{|r|c|c|c|c|c|c|c|c}
%    	
%    \hline
%     \multicolumn{1}{|c|}{\multirow{2}[2]{*}{\textbf{Classifier}}} &  \multicolumn{3}{c|}{\textbf{Political}} & \multicolumn{3}{c|}{\textbf{Non Political}} & \multirow{2}[2]{*}{\textbf{Macro-F1}}  \\
%    
%                 & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \\
%
%\multicolumn{1}{|l|}{\textbf{CNN}} &  \boldmath$0.97 (\pm 0.01)$ & \boldmath$0.91 (\pm 0.03)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.91 (\pm 0.03)$ & \boldmath$0.97 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
%
%\multicolumn{1}{|l|}{\textbf{SVM}} &  \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.93 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
%\multicolumn{1}{|l|}{\textbf{L. Regression}}  & \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
%
%  \multicolumn{1}{|l|}{R. Forest} &  $0.95 (\pm 0.01)$ & $0.89 (\pm 0.01)$ & $0.92 (\pm 0.01)$ & $0.89 (\pm 0.01)$ & $0.95 (\pm 0.01)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.01)$ \\
%  
%  \multicolumn{1}{|l|}{\textbf{N. Bayes}}  & \boldmath$0.91 (\pm 0.02)$ & \boldmath$0.99 (\pm 0.01)$ & \boldmath$0.95 (\pm 0.01)$ & \boldmath$0.98 (\pm 0.01)$ & \boldmath$0.90 (\pm 0.02)$ & \boldmath$0.94 (\pm 0.01)$ & \boldmath$0.94 (\pm 0.01)$ \\
%  
%  \multicolumn{1}{|l|}{G. Boosting}  & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.02)$ & $0.92 (\pm 0.01)$ & $0.92 (\pm 0.01)$ \\
% 
% \hline
%    \end{tabular}%
%  \label{tab:text_and_images}%
%  
%  
%\end{table*}%



==> WWW-CONF 2/5-analysis-political-ads.tex <==
\section{Analysis of political ads}
\label{sec:results}

In this section we investigate how many political ads our classifier
identifies in the \adanalystbr dataset. 
From \adanalystbr we removed
the ads that are part of the \gs dataset and were used for training the models, as well as the ads that we collected outside the election period (March 14, 2018 to August 15, 2018). We also removed  ads that were not in the Portuguese language, resulting in a set of 58,235 unique ads.
Finally, some advertisers create sets of ads that have the same text but with different images. In order to not over-represent them we only kept one ad for each set of ads with multiple images and the same caption. Hence, this leads us to a set of 38,110 ads. Remember that this dataset does not contain any official political ad as our browser extensions did not collect these ads (see Section~\ref{sec:dataset}).

%\footnote{In this section whenever we refer to the \adanalystbr dataset we mean the \adanalystbr dataset minus the \gs dataset.} 

We use the CNN model to assign to each ad a probability of being political.
In practice there is a significantly higher number of non-political
ads then political ads (i.e., we have an unbalanced dataset scenario). To limit the number of false positives (i.e., ads that are misclassified as political by our model but are actually non-political) we choose a threshold for declaring an ad as political that corresponds to a 1\% false positive rate (instead of choosing the typical 0.5 threshold for the probability of being political, which corresponds to a false positive rate of 8\% and true positive rate of 96\%). Using a threshold of 0.97, our CNN model classifies 835 ads as political out of the 38,110 ads we tested -- 2\% of the ads are political. The 835 ads were posted by 577 advertisers. 
We name the set of political ads we detect as the \polads. Figure~\ref{fig:ad_sample2} shows an example of such ad. We see that the ad mentions the name of a candidate and his identification number during the election.

To be sure the ads we detect are indeed about political issues we picked a random sample of 300 ads that were targeted by 251 advertisers and we manually check them. We found 19 ads that are not political and 2 ads we are not sure. The ads that were wrongly classified as political had captions that could mostly be easily confused by an algorithm; for example an ice-cream shop was presenting their products as mock-candidates in the election. %\thanos{the example is a bit extreme, but overall it got connfused by words like vote e.t.c}

This results suggest that at least 2\% of the ads in our dataset contain political content and are not part of the Facebook Ad Library. Note that our threshold for declaring political ads was very high and there might be many other political ads we do not detect due to this high threshold.  
This means that although a law exists to enforce the disclosure and registration of political ads on Facebook during the elections, there is still a considerable amount of political ads being broadcast that are not disclosed properly. 


\begin{figure}[t]
\includegraphics[width=0.9\columnwidth]{figures/ad_sample3.png}
\caption{Ad text posted together with this ad image translated to English: \normalfont{I am meeting friends, making new friends and bringing my message as a state deputy candidate to all residents of Marmelópolis (MG). Let's go together! A NEW LOOK FOR MINDS Political Advertising: CNPJ 31.208.669/001-05 \#Marmelópolis \#ANewLooking ForMines \#DrRobertoBob20200.}}
\label{fig:ad_sample2}
\end{figure}



%Since we cannot guarantee that our \Fbdata dataset is complete we cannot guarantee that all the ads that are not in \Fbdata are not part of the Facebook Ad Library. To further check if these ads are not part of the Ad Library, for each ad in \polads we query the Facebook Ad Library using the ad id we have in our dataset. \oana{@Thanos can you add a description of how you check this?} \oana{Our additional check shows that fill in the results}

\vspace{2mm}
\noindent \textbf{Compliance with the Brazilian election law:} 

%\vspace{2mm}
\noindent \textit{Disclosure:} We observed that some advertisers, even if they do not declare their ad as political on Facebook, they mention in the text of their ad the keywords ``Propaganda Electoral'' or ``Propaganda Política'', and their CPF or CNPJ tax id numbers, as required by the Brazilian law. We identified 90 such ads coming from 53 advertisers in \polads. 
While, these advertisers comply with the Brazilian election law, their ads are not declared to Facebook and, hence, are not  part of the Facebook Ad Library, thus evading future scrutiny. Note that, we have not checked if any of these advertisers declared their spending to the electoral court, to verify if the whole process is compliant.  % Hence, it is harder to audit them.  


%\textit{Posting time:} 
%No one is allowed to post political ads in the electoral period, which is around 1-month before the first voting round.  We identified \update{$703$} advertisers who did not follow these rules and placed ads with political content during the electoral period.
%\oana{this number does not seem right, because we only have 835 political ads; this would mean that each advertiser only posted 1 } \oana{mention the number of ads and the number of advertisers}
%\oana{how many advertisers?}

\vspace{2mm}
\noindent \textit{Type of advertiser:} 
Only political parties and politicians were allowed by law in Brazil to launch political ads during the electoral period, which is the period considered in our analysis. %We identified 577 advertisers in the \polads dataset.  
We manually checked who posted each ad from our sample of 300 ads. Out of the 232 advertisers who posted clear political ads, we detected 15 advertisers that are news organizations, and 28 advertisers that were neither news organizations, nor political parties or politicians. %\oana{so the rest is politicians and political parties?} 

Many of these advertisers --especially news organizations-- frequently covered news, debate events, interviews e.t.c., however, we  also identified 21 ads (from 12 advertisers) whose message was directly related to politics, often clearly advocating political agendas. For example, an NGO named \emph{Sou Da Paz} was advocating through 9 ads for several agendas related to reducing gun violence, crime rates e.t.c., while a community named \emph{Esquerda Marxista} placed 2 ads with heavy ideological undertone, one of which directly criticized Jair Bolsonaro. Table~\ref{tab:ads_sample} shows a (translated) ad for each of the two advertisers (AD5 and AD6, respectively).

% For the first:"Já está definido que haverá segundo turno para o próximo presidente da República e para governadores de alguns estados. O candidato que você vai votar propõe o que para transformar a situação caótica que estamos vivendo? Ele sugere soluções reais para que os responsáveis por crimes contra a vida sejam identificados e punidos?   Só vamos conseguir acabar com a impunidade se valorizarmos o trabalho das polícias. Para melhorarmos a investigação, são necessárias ações como o estabelecimento de metas estaduais de redução de mortes violentas e investimento em equipamentos e técnicas de perícias criminais. Saiba mais sobre essa e outras propostas para transformar essa realidade na agenda  # SegurançaPúblicaÉSolução :  http://bit.ly/ResumoSegurançaPúblicaÉSolução   # NãoTáTudoBem   # DáPraResolver", 

% and second  "A luta contra Bolsonaro só pode ser efetiva se encarada como parte da luta da classe trabalhadora contra o atual sistema. Venha conhecer o combate dos comunistas.  # ElesNão : Bolsonaro e os demais representantes do capital"

% \oana{@thanos, put your analysis, mention out of the sample you manuyally labeled, how many are news medias, how many are not politicians}


\vspace{2mm}
\noindent \textit{Representation in the Ad Library:} The ads in \polads were not declared as political on Facebook and hence are not part of the Ad Library.  To check whether there might be versions of these ads that are part of the Ad Library, for each ad in \polads we extract the text of the ad and we check if the text matches any of the ads in the \Fbdata dataset. Only 34 of the 835 ads have a corresponding ad in \Fbdata.
This shows that for a small fraction of ads, the advertisers had some ads that were compliant with the Facebook's ToS but also similar versions of the same ad that were not.

%(are the \polads part of the Facebook Ad Library?)

%Figure~\ref{fig:ads_intersection} illustrates the overlap between the \polads dataset and the official political Facebook ads from the \Fbdata dataset.






\vspace{2mm}
\noindent \textbf{Differences between ads in \polads dataset and the \Fbdata dataset:} 
In Table~\ref{tab:ads_sample} we show (translated) examples of ads from \Fbdata and \polads. % For the sake of comprehension, we translated all ads from Portuguese to English. 
%%\update{AD1 is an educational ad about the importance of creating a political sense from an early age. AD2 is a warning cry claiming that the congressman was expelled from Congress. It is not clear in the text of the ad why he was kicked out. AD3 is an educational ad promoting articles and videos that explain election myths. Its main point is to demystify rumors that arose during Brazilian elections. AD4 is a typical political ad where the candidate talks about issues like security, abortion, racism and public health. In AD5, the candidate invites people to join his WhatsApp group. During 2018 Brazilian elections the WhatsApp was massively used to spread political and ideological content, mainly because of the difficulties involved in tracing and punishing bad conduct. Similar to AD4, adds AD6, AD7, and AD8 describe candidates explicitly asking for votes, but unlike AD4, these ads are not official political ads. Finally, AD9 is another typical political ad where the candidate asks for votes, but in this case, this ad was collected by our system and is also an official political ad.}\thanos{if we need to cut something we can cut this, or summarize it in one sentence. The next paragraph is enough} \oana{I agree we can cut all the colored text}
We do not see a clear distinction among ads of each group as they both contain explicit publicity material for candidates as well as ads related to the elections but not to particular campaigns. This sample of examples illustrates  the importance of having collaborative systems that enable the participation of the society on the process of uncovering (potentially suspicious) political campaign actions.
%One would expect that ads in \Fbdata would describe a political agenda much more clearly than the ones belonging to\polads, but this is not the case. 
% In \Fbdata ads contain explicit publicity material for candidates (AD1, AD2, AD3 and AD4) and ads related generally to election but not related to a particular political campaign (AD5, AD6, AD7 and AD8)\thanos{I don't understand the point here}. 
%\update{Overall, we notice that \Fbdata ads tend to contain explicit publicity material for candidates while \polads include also ads related to the elections but not only to particular campaigns.} \oana{ it is a bit weird to say that we want to detect ads similar with the ones in the ad library but we end up with ads that are a bit different}
%\thanos{made a small edit because it was not super clear(see the comments), but are we sure about that for \Fbdata?)}


%\thanos{@marcio: for what purpose do we do that? For the website? In the next paragraph we say that we use the 90\% threshold.}. 

%This is a problem, because we decided that it is important that the list of political ads shown by the system does not contain, if possible, a single false positive ad. Thus, with the help of the ROC curve shown in Figure~\ref{fig:roc_result}, we decided to increase this threshold to \change{$95\%$}, what leads to a false positive rate of only \change{$7.6\%$} and true positive rate of \change{$7.8\%$}, still a considerably high value. With this threshold, our system is able to still retrieve a good amount of political ads from the database and, more important, we can be very confident that these ads are indeed political. 


%To illustrate the potential of our system, let us consider the following question: \textit{what is the fraction of advertisers in our database who sponsored political ads and were not part of \update{the political advertisers that we collected from Facebook Ad Library?}} Recall that only political parties and politicians were allowed by law in Brazil to launch political ads during the electoral period, which is the period considered in our analysis.  
%To be very conservative in answering this question, next we choose an even stricter threshold, $90\%$, for the chance of an ad to be political.
%Figure~\ref{fig:adv_intersection} shows that \textbf{only} \update{259 out of 1,303 ($\approx 19.87\%$)} advertisers who sponsored political ads were listed as \update{political advertisers in Facebook Ad Library}. Note that \update{$1,303$} is the number of advertisers who sponsored at least one ad inferred as ``political'' by our system, i.e., an ad that was classified as ``political'' using the $50\%$ threshold. 

%Similarly, Figure~\ref{fig:ads_intersection} illustrates the fraction of ads listed as ``political'' by our system that was not properly targeted as such in the Facebook ad platform. Observe that \textbf{only} \update{$87$ out of 1,679 ($5.18\%$)} ads were official political ads. Recall that \update{$1,679$} is the number of ads that were listed as ``political'' by our system, i.e., an ad that was classified as ``political'' using the $50\%$ threshold (Our \update{$233$ political ads previously labeled are not subset of these $1,679$}). Results depicted in Figures~\ref{fig:adv_intersection} and~\ref{fig:ads_intersection} reveal a striking fact: although a law exists to enforce the disclosure and registration of political ads on Facebook during the elections, there is still a considerable amount of political ads being broadcast that are outside this law.\thanos{need to check these ads manually before we make such a claim)}

%The first question we needed to answer: \emph{Is there an intersection between advertisers who sponsored ads and were collected by AdAnalyst plugin and Advertisers who sponsored official political ads?}

%\begin{figure}[ht]
%\includegraphics[width=0.5\columnwidth]{plots/adv_intersection_v3.png}
%\caption{Advertiser intersection (\emph{C}) between Official Advertisers (\emph{A}) and Plugin Advertisers (\emph{B}).}
%\label{fig:adv_intersection}
%\end{figure}

%Finally, what about the ads which these advertisers sponsored: \emph{Is there an intersection between ads which were collected by AdAnalyst plugin and official political ads?}

%\begin{figure}[ht]
%\includegraphics[width=0.5\columnwidth]{plots/ads_intersection_v3.png}
%\caption{Ads intersection (\emph{C}) between Official Ads (\emph{A}) and Plugin Collected Ads (\emph{B}). \oana{remove the black circle; use the color blue instead of yellow -- not sure if it looks good when printed in Bblack and white}}
%\label{fig:ads_intersection}
%\end{figure}





% Those ads should be declared on Facebook as political so that those ads could go to the Facebook archive and the money spend on them could be made transparent to society. Those ads in group B are ads bypassing the Facebook approach to provide transparency and potentially bypassing the Brazilian law who trusted Facebook to identify those ads. Our system unveiled dozens of similar ads from group B. 

%\newpage 
%\marcio{Dont worry, I will fix this table to fit in two columns }
\begin{table*}[t]
%\begin{longtable}[!htb]{ |p{0.5cm} |p{10cm}|p{5.4cm}|}
\caption{Sample of ads in \Fbdata and \polads.}
\label{tab:ads_sample}
\begin{small}
\begin{tabular}{ |p{0.5cm} |p{12.5cm}|p{3.5cm}|}
%\multicolumn{3}{|c|}{Sample Ads} \\ 
\hline
\# & Ad Text & Ad and Advertiser Info \\
\hline
\multicolumn{3}{c}{\Fbdata} \\
\hline
AD1 & The candidate Romeu Zema, tried once again, to hitch a ride in the campaign of Jair Messias Bolsonaro. This time he didn't make it, because people have already started to discover who he really is. \#eleicoes2018
%O candidato Romeu Zema, tentou mais uma vez, pegar carona na campanha de  Jair Messias Bolsonaro . Dessa vez ele não conseguiu, pois as pessoas já começaram a descobrir quem ele realmente é.  #eleicoes2018
& Public Figure

fb.com/deputadomarcosmontes
 \\ \hline
 AD2 & 3 days to go! It was an incredible journey to get here receiving affection and support from so many people. Check out the retrospective of my campaign and don't forget: on October 7, vote 2332 for Deputado Federal RJ. I count on you! bit.ly/2P8kkxz
%Faltam 3 dias para as Eleições! Foi uma jornada incrível chegar até aqui recebendo carinho e apoio de tanta gente. Confira a retrospectiva da minha campanha e não se esqueça: no dia 7 de outubro, vote 2332 para Deputado Federal RJ. Conto com você!  bit.ly/2P8kkxz
&Public Figure

fb.com/FlavioCavalcantiJunior
\\ \hline
AD3 & It is a great satisfaction to receive the support of Carlos Roberto Osorio. He will not run for reelection, but he demonstrates that he has better security in Rio. Vote 40021 for state deputy - Renan Ferreirinha
%É uma grande satisfação receber o apoio do Carlos Roberto Osorio. Ele não irá concorrer à reeleição, mas ele demonstra que tem esperanças de um Rio melhor. Vote 40021 para deputado estadual - Renan Ferreirinha
& Politician

fb.com/RenanFerreirinha/

\\ \hline 
AD4 & Friends, in this final phase, I need your support! Anyone who has always followed my work knows that I did a lot, but as \#DeputadoEstadual I can do even more. Have you ever chosen11222 help me share it with your friends and family? \#AForçaDoInterior  \#NewPolicy \#WellPolicy \#CleanFile
& Politician

fb.com/fabiomanfrinatobauru/
\\ \hline


\multicolumn{3}{c}{\polads} \\
\hline
AD5 & 
Proposal of Agenda \#SegurançaPúblicaÉSolução: end impunity! Only increasing penalties does not solve impunity: of what use a hundred years worth if the person responsible for the crime is not arrested? The work to change that is to invest in research well made, which identifies criminals, dismantle gangs and arrest those who commit violent crimes such as murder and rape. \#NãoTáTudoBem \#VamosResolver? Meet this and other proposals to improve public security in Brazil: http://bit.ly/ResumoSegurançaPúblicaÉSolução
%Proposta da Agenda  # SegurançaPúblicaÉSolução : acabar com a impunidade!  Só aumentar penas não resolve a impunidade: de que adiantam cem anos de pena se a pessoa responsável pelo crime nem é presa? O trabalho para mudar isso é apostar na investigação bem feita, que identifica criminosos, desmonta quadrilhas e prende quem comete crimes violentos como homicídios e estupros.  # NãoTáTudoBem   # VamosResolver ?  Conheça essa e outras propostas para melhorar a segurança pública do Brasil:  http://bit.ly/ResumoSegurançaPúblicaÉSolução   
& NGO


\url{fb.com/institutosoudapaz/}

\\ \hline

% AD5 & 
% Son of Mrs. Maria 1st Deputy Councilman 1,930 votes President. Assoc. of Residents of Guabiroba Sec. Parliamentary of the Chamber of Deputies!
% %Filho da dona Maria 1º Suplente de Vereador 1.930 votos Presidente. Assoc. de Moradores da Guabiroba Sec. Parlamentar da Câmara dos Deputados!
% & Community


% \url{fb.com/cesinhaOfficial/}

% \\ \hline

AD6 &
The fight against Bolsonaro can only be effective if seen as part of the struggle of the working class against the current system. Come to know the fight of the Communists. \#ElesNão: Bolsonaro and other representatives of capital.
%A luta contra Bolsonaro só pode ser efetiva se encarada como parte da luta da classe trabalhadora contra o atual sistema. Venha conhecer o combate dos comunistas.  # ElesNão : Bolsonaro e os demais representantes do capital
& Community

\url{fb.com/EsquerdaMarxista/}
\\ \hline
% AD6 &
% \#EDITAL - Against current setbacks, we need to stir up our thoughts and react to transform society. In this sense, FASE's SAAP Fund has an open call for proposals to support training activities and political advocacy in peripheral areas and \#favelas across the country. We believe it is important for organizations, groups and collectives to articulate themselves in order to build narratives that recover, expand and strengthen processes of social mobilization and \#political action. Participate: https://bit.ly/2NOeKPI
% %#EDITAL - Contra os atuais retrocessos, precisamos agitar os pensamentos e reagir para transformar a sociedade. Nesse sentindo, o Fundo SAAP, da FASE, está com um edital aberto para apoiar ações de formação e incidência política em áreas de periferia e #favelas de todo o país. Acreditamos ser importante que organizações, grupos e coletivos se articulem para a construção de narrativas que recuperem, ampliem e fortaleçam processos de mobilização social e ação #política . Participem: https://bit.ly/2NOeKPI
% & ONG

% \url{fb.com/ONGFase/}
% \\ \hline
AD7 & 
[ELECTIONS 2018 - INTERVIEW WITH BISHOP DAMASCENO] Continuing the interviews of the Luziense Observatory with candidates from Santa Luzia in the 2018 Elections, we talked with the city candidate for Senate, Bishop Damasceno, of the PPL. Check out! \#elections2018 \#interview \#senado \#bispodamasceno \#politics \#TVOL \#santaluzia \#observatorioluziense \#luziar
%[ELEIÇÕES 2018 - ENTREVISTA COM BISPO DAMASCENO] Dando prosseguimento às entrevistas do Observatório Luziense com candidatos de Santa Luzia nas Eleições 2018, conversamos com o candidato da cidade ao Senado, Bispo Damasceno, do PPL. Confira! #eleições2018 #entrevista #senado #bispodamasceno #política #TVOL #santaluzia #observatórioluziense #luziar
& News Media


\url{fb.com/observatorioluziense/}
\\ \hline
AD8 & Hi, Hi Dear People! For state representative, vote Luiz Carlos Martins - 11550!%Oi, Oi Gente Querida! Para deputado estadual, vote Luiz Carlos Martins - 11550!
& Politician



\url{fb.com/luizcarlosmartinsoioi/} \\ \hline
% AD8 & The rescue of morality is the initial step so that we can reconstruct the State of Rio de Janeiro, with legitimate representatives of the people, in the figure of men who act with principles and who, above all, carry with them, victims such as ETHICS and JUSTICE. %O resgate da moralidade é o passo inicial para que possamos reconstruir o Estado do Rio de Janeiro, com legítimos representantes do povo, na figura de homens que ajam com princípios e que, acima de tudo, carreguem consigo, viturdes como a ÉTICA e a JUSTIÇA.
% & Politician 

% (\url{fb.com/Fernando-Sauerbronn-Estadual-17700-307295073185943/}) \\ \hline



%AD9 &
%Do not fall into speeches with empty promises. A strong economy is the basis of everything. \textit{\#ChamaOMeirelles \#VoteMeirelles15}
%Não caia em discursos com promessas vazias. Uma economia forte é a base de tudo. \#ChamaOMeirelles \#VoteMeirelles15 
%& Politician 

%\textbf{Facebook Page:}  

%(\url{fb.com/hmeirellesoficial/})

%\textbf{Ad Group}: C
%\\ \hline

\end{tabular}
\end{small}
\end{table*}
%\end{longtable}\label{tab:ads_sample}

%\newpage

%\begin{figure}[t]

%\includegraphics[width=0.9\columnwidth]{figures/ad_sample1.png}
%\caption{Ad text posted together with this ad image translated to English: \normalfont{Anastasia recognizes the work of Antonio Jorge! \#AJ23123.}}
%\label{fig:ad_sample1}
%\end{figure}



%that should appear in the Facebook archive. It is important to highlight this group of ads, as along the period we considered in our analysis, only Brazilian politicians and political parties were allowed by law to make political ads on Facebook. Such ads, that potentially bypass the related legislation, can be observed frequently in group B. However, ads not in regulatory compliance can be found in A or B if their advertisers does not declare their spending to electoral court.


%Figures \ref{fig:ad_sample1} and \ref{fig:ad_sample2} show examples of ads from group B. We see that these ads mention the name of candidates or their \update{identification number during the election}, and are clearly political ads that should appear in the Facebook archive. It is important to highlight this group of ads, as along the period we considered in our analysis, only Brazilian politicians and political parties were allowed by law to make political ads on Facebook. Such ads, that potentially bypass the related legislation, can be observed frequently in group B. However, ads not in regulatory compliance can be found in A or B if their advertisers does not declare their spending to electoral court.




%\oana{cut? I do not see how the sample is making this point}

%\update{This sample of examples illustrates the difficulty of tracking illegal political ads on social media platforms, which is corroborated by \cite{wong2013quantifying}, and the importance of having collaborative systems that enable the participation of the society on the process of uncovering suspicious political campaign actions.
%} \oana{cut? I do not see how the sample is making this point}


 %\end{longtable}
 


==> WWW-CONF 2/6-related-work.tex <==
\section{Related Work}\label{related-work}

Social networks rise as a new battlefield during elections and the Facebook ad platform was shown to be quite effective in many marketing segments, including political advertising.\footnote{ https://www.wordstream.com/blog/ws/2017/02/28/facebook-advertising-benchmarks} %However, the abundance of targeting attributes that Facebook provides to advertisers have been raising concerns about its use for political campaigns~\cite{russian-ads} as well as its potential to create discriminative ads~\cite{speicher-2018-targeted}.
We review related efforts along four axes: (i) studies related to sentiment analysis on political content, (ii) studies focused on Facebook ads, (iii) studies on the relationship between social media and the general public, and (iv) studies on the social media influence on election results.

%\emph{Political sentiment analysis}.
\vspace{2mm}
\noindent{\textbf{Detection of political content and sentiment.}}
Durant \textit{et al.}~\cite{Durant2007} implemented automatic techniques that identify the political sentiment of web blog posts and help bloggers categorize and filter this exploding information source. Bakliwal \textit{et al.}~\cite{bakliwal2013sentiment} also implemented a classifier for sentiment analysis, but they have not detected political content, only sentiments. In contrast, Oliveira \textit{et al.}~\cite{oliveira2018} built a CNN (Convolutional Neural Network) for detecting political tweets from a collection of $2,000$ congressmen tweets labeled as \textit{political} and \textit{non-political}. 

%\emph{Facebook Ads}.
\vspace{2mm}
\noindent{\textbf{Analysis of Facebook ads.}}
Andreou \textit{et al.}~\cite{andreou2018investigating} investigated the level of transparency of Facebook explanations and showed that the Facebook ad explanations are often incomplete and sometimes misleading, while data explanations are often incomplete and vague. In addition, Andreou \textit{et al.}~\cite{Andreou19a} characterized advertises on Facebook. They found that a non-negligible fraction of advertisers belongs to sensitive categories such as news and politics, and that there exist many niche, unverified advertisers whose trustworthiness is difficult to estimate in an automated way. Also, their analyses revealed that a significant amount of advertisers use targeting strategies that can be characterized as invasive or opaque. In a related work, Speicher \textit{et al.}~\cite{speicher-2018-targeted} showed that a malicious advertiser can create highly discriminatory ads without using sensitive attributes.

%\emph{External ads influence}.
%\vspace{2mm}
%\noindent{\textbf{Political ads.}}
Recent papers studied how Russian ads were able to affect U.S. citizens. Ribeiro \textit{et al.}~\cite{ribeiro2019@fat} investigated how malicious Russian advertisers were able to run ads with divisive or polarizing
topics (e.g., immigration, race-based policing) at vulnerable subpopulations. Authors have analyzed divisiveness of the ads based on topics that caused different reactions among different social groups. Kim \textit{et al.}~\cite{kim-pol-com2018} used an ad tracking app that enabled them to trace the sponsors/sources of political campaigns and unpack targeting patterns. Their empirical analysis identified ``suspicious'' groups, including foreign entities, and operating divisive issue campaigns on Facebook.
Etudo \textit{et al.}~\cite{etudo2019facebook} also investigated the effects of Russian ads and what is the relation with Black Lives Matter Protests. The study found that Russian ads related to police brutality were issued to coincide with periods of higher unrest.


%\emph{Social media and general public}.
\vspace{2mm}
\noindent{\textbf{Influence of social media on the general public.}}
Concerning the role of social media on the general public, Wang and Mark \cite{Wang:2017} studied how college students engage with political and social issues on Facebook and found that the impression management and disclosure concerns strongly influence some people to refrain from commenting or sharing content. However, there is evidence that social media can create a public sphere that enables discussions and deliberations~\cite{Maruyama2014}. For instance, Kou et. al. \cite{kou2017one} analyzed the public discourses about Hong Kong’s Umbrella Movement on two distinct social media sites, Facebook and Weibo. They show how people on these two sites reasoned about the many incidents of the movement and developed sometimes similar but other times strikingly different discourses. 

Despite enabling public discourse, social media can leverage some problems such as biased content. For example, Kulshrestha \textit{et al.}~\cite{Kulshrestha:2017} proposed a framework to quantify bias in politics-related queries on Twitter. They found that both the input data and the ranking system contribute significantly to produce varying amounts of bias in the search results, what can have a significant impact on the impression that users form about the different events and politicians. Similarly, Gao \textit{et al.}~\cite{Gao:2018} conducted a controlled experiment to study how stance labels to separate news articles with opposing political ideologies help people explore diverse opinions. Results show that stance labels may intensify selective exposure - a tendency for people to look for agreeable opinions – and make people more vulnerable to polarized opinions and fake news.

These latter two topics are problems analyzed by Che \textit{et al.}~\cite{Che:2018}, who compared and contrasted the ways left- and right-wing news organizations treat the concept of fake news in the context of the highly polarized nature of U.S. news media as well as the evolving and nebulous nature of fake news. They found some key differences. While left-leaning sources discuss specific examples of fake news, the narrative in right-leaning sources focuses on mainstream media as a whole. Moreover, Garimella \textit{et al.}~\cite{Garimella:2018} showed that people who try to bridge the echo chambers, by sharing content with diverse leaning, have to pay a ``price of bipartisanship'', which is a latent phenomenon that effectively stifles mediation between the two sides.


%\emph{Social media influence on election results}.
\vspace{2mm}
\noindent{\textbf{Influence of social media on election results.}}
There is already evidence that the action and interaction of voters in social media can influence their inclination to vote or not for a candidate. Maruyama \textit{et al.}~\cite{Maruyama2014} found a relation between Twitter use and the voting choice. They investigated how using a social network while watching a political event could influence the experience of a voter, especially when the user actively participates by posting messages about the event. Pal \textit{et al.}~\cite{pal2018speaking} examined the function and public reception of critical tweeting in online campaigns of four nationalist populist politicians during major national election campaigns. They found that cultural and political differences impact how each politician employs their tactics.
However, politicians are not only the ones who try to influence the elections. Hemphill and Roback \cite{Hemphill2014} examined hundreds of citizen-authored tweets and the development of a categorization scheme to describe common strategies of lobbying on Twitter. Contrary to past research, they found that assumed citizens used Twitter to merely shout out their opinions on issues and utilize a variety of sophisticated techniques to impact political outcomes. Finally, \citet{tumasjan2010predicting} investigated whether Twitter is used as a forum for political deliberation and whether online messages on Twitter validly mirror offline political sentiment. They concluded that the mere number of messages mentioning a party reflects the election result in the German federal election.

Regarding the behavior of politicians in social media, Hwang \cite{Hwang2013} analyzed how Korean young adults evaluate the use of Twitter by South Korean politicians, perceive politicians' credibility, and evaluate politicians who use Twitter. The author concludes that politicians who actively use Twitter are seen as more credible and, as a consequence, are more positively evaluated by young adults.
Still in South Korea, Lee and Shin~\cite{Lee2012} and Lee \textit{et al.}~\cite{Lee2014} designed experiments to investigate how the level of interactivity in politicians' Twitter communication affects the public's cognitive and affective reactions. They found that exposure to high-interactivity Twitter pages induce a stronger sense of direct conversation with the candidate, which, in turn, led to more positive overall evaluations of the candidate and a stronger intention to vote for him. %Persily~\citet{persily20172016} discuss about the 2016 USA Election and heavy use of social network which led Donald Trump winning votes. 
%Indeed, social networks rise as important tools for candidates connect with their voters. Additionally, Facebook ads is a good way to stick the social bubble and spreading political content to specific set of users, by micro-targeting. 

Our work is novel in many aspects and provides complementary insights to the discussed studies. 
We focus on detecting political content in advertisement with the aim of monitoring the misuse of Facebook ads platform. Our paper highlights the importance of independent auditing platforms for political ads and our effort provides all the necessary framework to make it feasible. 




==> WWW-CONF 2/7-conclusion.tex <==
\section{Concluding Discussion} \label{sec:conclusion}

%\oana{even with a method trained on only a few examples we were able to detect much more political ads than facebook}
In this work we presented a system for detecting political ads in Facebook and which we deployed during the Brazilian 2018 elections\footnote{https://www.eleicoessemfake.dcc.ufmg.br/anuncios/}.
%Among our main contributions, we compared the ads detected by our algorithm with the ads labeled as political in the Facebook ad archive. 
Although we have only a small sample of the ads running in Facebook, our approach was able to identify many ads with political content that are not part of the Facebook Ad Library for political ads. 
The main culprit for this situation is that advertisers need to self-declare their political ads as such for them to appear in the Ad Library. It is not clear whether Facebook has any mechanism to enforce compliance. 

The Brazilian election legislation stipulates that ads during the electoral period need to be labeled with the \emph{Propaganda Electoral} tag display the national identification number (CPF for individuals and CNPJ for institutions) of the advertiser. A small fraction of advertisers in our dataset have the right disclaimer stipulated in the Brazilian election law but they did not declare their ads as political to Facebook, hence, they do not appear in the Ad Library.

%Along the Brazilian election, only politicians and political parties were allowed by law to promote political ads on Facebook. Also, those ads should be declared as political and should 
%With that, ads can go to the Facebook archive and the money spent on them, as well the advertisers, can be transparent to the society. 

% Our system revealed a number of ads that were not properly declared as political by the advertiser, potentially bypassing the Facebook interface to regulate them and, consequently, the Brazilian law. 

While the results in our paper are undeniably worrying as there are Brazilian advertisers that did not declare their political ads, there is a positive side to it: we were able to exploit the ads self-declared as political from compliant advertisers to build machine learning-based models that can detect other similar ads coming from advertisers that do not comply with the Facebook's ToS or electoral laws. 

One limitation of our work is that our results refer exclusively to the Brazilian scenario. We only tested machine learning-based models trained on ads in Portuguese and evaluated them only on ads during the 2018 Brazilian elections.  Assessing the accuracy of such techniques on ads in other languages and testing how well these techniques are adapting to future elections remains an open question. 
Because of that, we plan to analyze other elections using the methodology described in this paper and our browser extension continues to be live (\url{https://adanalyst.mpi-sws.org/}). 

%We understand that it might be hard for Facebook to deal with the problem of deploying an ad detection algorithm per country or even prohibiting the promotion of political ads at all, an extreme measure adopted by Twitter on October 29, 2019 based on their belief that political message reach should be earned, not bought.  

We hope our findings and all the real-world experience of deploying a real system along the 2018 Brazilian elections will inform debates around public policies that regulate political advertising on the Internet. % and open the discussion among academics, public servants and the society is the path for a global solution to the problem.
If a system like ours is implemented on a widespread scale, political campaigns might adopt adversarial strategies that change their marketing strategies in order to exploit our false negative rate. The existence of multiple independent auditing systems would make the monitoring of political ads more robust to attackers. We hope our effort will inspire other initiatives around the world.  Our paper not only highlights the importance of independent auditing platforms for political ads but also provides all necessary framework to make it feasible as our code is open source.
%On our side, we hope that exploring solutions along different elections and countries and





%we focus only on the text  associated to the ads, without exploring the content of videos and images, which we left for future work.  Another limitation is that



%It is possible that our effort and the changes deployed by Facebook along the Brazilian elections have made the misinformation campaigns to adapt their strategies and migrate to other social networks and communication systems. Unfortunately, the Brazilian 2018 elections were still marked by the abuse of misinformation campaigns, which found in WhatsApp a fertile ground\footnote{https://www.bbc.com/news/technology-45956557}. 

%\change{In light of this limitation, we plan to expand this work to other social media platforms, including WhatsApp. Another limitation of our work is that our results refer exclusively to the Brazilian scenario. Because of that, we plan to analyze other elections, such as the one in India and in the UK, using the methodology described in this paper.  }

%thus, we will not be able to detect them. These techniques constitute usual behavior when advertisers place ads with products or content prohibited on Facebook. 



\if 0

\oana{text copied from other places that could fit in clonclusion}

\update{ Our study also shows the importance of having access to archives of self declared political ads. These ads are essential for training machine learning-based algorithms that can discriminate automatically between political and non-political ads. }

%So, beyond \datasetBrazil, we need to improve our model training with more data provided by Facebook, containing rich data about non-political ads, and not only political ads and national issues as it provides today. 
%\oana{I really like this point, having more independent auditing systems it is more robust to attackers}


\update{One of the key issues with the current approach from Facebook, is that it relies on advertisers to self-declare their political ads as such. 
Our system is to be able to identify at least a set of political ads that were not properly declared as political by the advertiser, thus being potentially not in Brazilian regulatory compliance.}


\update{In another hand, on October 29, 2019, Twitter globally prohibited the promotion of political content. They have made this decision based on their belief that political message reach should be earned, not bought}. 

\fi 

==> WWW-CONF 2/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> WWW-CONF 2/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> WWW-CONF 2/backup-4-classifier.tex <==
\section{Detecting political ads} \label{sec:methodology}

 In this section we describe our approach to identify political ads. This approach has three steps. First, we create a gold standard collection of ads used to test our method. Then, we select a supervised classifier that receives as input the text of an ad and outputs if it is political or non-political. Finally, we evaluate this classifier over different sets of training data.

\subsection{Gold Standard Collection}\label{sec:labeling-ads}

 To appropriately train and test our model, we needed a dataset with the same statistical properties as the ones we find in production, i.e., when the system goes online. The \textit{Official Political Facebook Ads} contains only political ads and the \textit{Twitter dataset} does not contain any ad, only tweets. Thus, we construct our \textit{gold standard collection} from the \textit{AdAnalyst dataset}, as the amount of political and non-political adds are distributed according to what users see in their feeds.

 From the $239K$ unique ads of this dataset, we sampled $10,000$ to be labeled by three independent volunteers. Their job is to label each ad of this sample as \textit{political} or \textit{non-political} according to Definition~\ref{def1}. We evaluate the inter-rater reliability among the independent volunteers  using the agreement percentage and the Cohen's Kappa coefficient ($\kappa$)~\cite{Oren2011,Landis1977,Savage2015}. This coefficient measures the agreement between two volunteers who each classify a predefined number of ads as one of the two mutually exclusive categories: \emph{political} or \emph{non-political}.

 From Table ~\ref{tab:labeled}, we observe that the agreement among the three volunteers is consistently high, 99.7\% for volunteers  1 and 2, with $\kappa = 0.93$, and 99.5\% for volunteers 1 and 3, with $\kappa = 0.88$. For volunteers 2 and 3 the agreement is 99.5\%, with $\kappa = 0.89$. According to Landis and Koch~\cite{Landis1977}, these Kappa scores fall into the range of scores referred to as ``Almost Perfect'' agreement, which is a satisfactory result that validates our \textit{gold standard collection}.

\begin{table}[ht]
\centering
\caption{Cohen's Kappa and Agreement percentage among researchers over \textit{labeled training set} containing $10,000$ Facebook ADs}

\label{tab:labeled}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
 & & \textbf{Researchers} \\
\hline
	&	\textbf{1 and 2}	&	\textbf{1 and 3} & \textbf{ 2 and 3} \\
\hline
Kappa coefficient $\kappa$	&	0.93	&	0.88	&   0.89 \\ 
Agreement \%			&	99.7\%	&	99.5\%  &   99.5\% \\
\hline
\end{tabular}
}
\end{table}

\subsection{Learning algorithms for automated detection of political ads}

 In a recent effort, Oliveira et al.~\cite{oliveira2018} proposed a successful Convolution Neural Network (CNN) architecture for identifying political tweets posted by politicians. Because of the similarity of their task with ours, we propose the use of the same architecture to identify political ads.

 Figure~\ref{fig:cnn_model} shows this architecture. In the input layer, we represent each word of a Facebook ad as a dense vector retrieved from Word2Vec C-BoW~\cite{Mikolov2013} with 300 dimensions, pre-trained over a large Portuguese data set \cite{Hartmann2017}, which is able to produce an embedding matrix for a vocabulary of 1.3 trillion words.
Thus, the input layer is a matrix $n \times 300$, where $n$ is the number of words in a particular ad and $300$ is the vector representation of each word of this message. Subsequently, there is a 25\% rate dropout regularization layer connected to a convolutional layer with $120$ different filters and sizes (3,4,5), activated by a ReLU function. Then, the output of the previous layer is connected to a global max-polling layer, whose output is, in turn, fully connected to a ReLU activation and to another 25\% rate dropout layer. Finally, the last dense layer is a single neuron with a sigmoid activation function that outputs $1$ if the message is \textit{political}, and $0$ if \textit{non-political}. Moreover, we optimized the neural network by means of cross entropy loss function using the RMSProp~\cite{Duchi2011} optimization algorithm.
 

\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\linewidth]{figures/cnn_model.pdf}
\caption{Convolutional Neural Network architecture for political Ads classification.}
\label{fig:cnn_model}
\end{figure*}
 
\subsection{Evaluation}

 \update{Our \textit{gold standard collection}, contains $233$ political and $9,767$ non-political advertisements manually labeled. In addition to this collection, we consider the another dataset described in Section~\ref{sec:dataset} for gathering textual features used to train and test our models:  the \textit{Official Political Facebook ads}, whose we randomly selected $10,000$ official political ads. Then, our train and test dataset has $20,000$ ads splitted in 10-\emph{folds}, $90\%$ for train and $10\%$ for test. In order to evaluate our choice of the classifier, we also run the results for four classic supervised baselines: Logistic Regression, Gradient Boosting, and Naive Bayes.}
 
 \update{In order to add extra textual feature to Lebaled Ads, we extracted texts from the all image in Labeled Ads, then we added to train. Our main goal adding these extra feature is investigated whether the model performance would be better than previous analysis without ad image features. In total, $7,598$ out of $10,000$ labeled ads had text. }

\if 0
\begin{table}[ht]
\small
  \caption{Text features for training and validation}
  \label{tab:features}
  \begin{tabular}{clccc}
    \toprule
    
    \textbf{Abbrv} & \textbf{Text feature} & \textbf{pol.} & \textbf{non-pol.} & \textbf{Total}\\
	
    \toprule
    $S1$ & Labeled Tweets  & $1,000$ & $1,000$ & $2,000$\\
    $S2$ & Labeled Facebook Ads & 233 & 9,767 & 10,000\\
    $S3$ & Official Political Facebook Ads\footnote{https://www.facebook.com/politicalcontentads} & \update{26,059} & 0 & \update{26,059}\\
  \bottomrule
\end{tabular}
\end{table}
\fi

As evaluation metrics, we considered two classic metrics: accuracy and Macro-F1. Accuracy considers equally important the correct classification of each ad, independently of the class, and basically measures the capability of the method to predict the correct output. A variation of F1, namely, Macro-F1, is normally reported to evaluate classification effectiveness on skewed
datasets.  Macro-F1 values are computed by first calculating F1 (a metric that captures both precision and recall) values for each class in isolation, then averaging over all classes. This way, Macro-F1 considers equally important the effectiveness in each class, independently of the relative
size of the class.

%In the training process we used $10$\emph{-fold} \emph{cross-validation}. 
%For each test fold $i$, we trained the model with the rest, until all folds have been used as test fold. Then, we calculate the mean and confidence interval for each class metrics (\emph{precision}, \emph{recall}, \emph{f1}), also \emph{Macro-F1}, \emph{AUC - Area Under the Roc Curve}  and \emph{accuracy}. 


\begin{table}[ht]
\centering
\tiny
\caption{Results obtained for different classifiers w.r.t
AUC and F1-macro score}

\label{tab:results_experiments}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\hline
 & \textbf{Metrics} &  \\
\hline
	&	\textbf{AUC}	&	\textbf{F1-macro}  \\
\hline
CNN 	        & $0.98 (\pm 0.010)$	& $0.94 (\pm 0.010)$ \\ 
SVM 			& $0.98 (\pm 0.010)$  & $0.94 (\pm 0.012)$ \\
L. Regression 	& $0.98 (\pm 0.014)$  & $0.94 (\pm 0.009)$ \\
R. Forest 		& $0.97 (\pm 0.012)$	& $0.92 (\pm 0.008)$ \\
N. Bayes 		& $0.99 (\pm 0.011)$  & $0.94 (\pm 0.009)$ \\
G. Boosting 	&$0.97 (\pm 0.019)$	& $0.92 (\pm 0.011)$ \\

\hline
\end{tabular}
}
\end{table}

%Also, we evaluate the classification performance of the each learning method considering each combination of textual features as input: $S1$, $S2$, $S3$, $S1 + S2$, $S1 + S3$, $S2 + S3$, $S1 + S2 + S3$. Our goal is to assess the discriminating power of adding each set of textual features and understand if adding features from tweets, for example, would add noise or help in differentiate political ads from the non-political ones.

%In Table~\ref{tab:tabelao2}, we show the results for all configurations of \textbf{input} and \textbf{method}. We highlight in bold all the configurations that achieved the statistically highest Macro-F1 scores. First, observe that using all datasets as input have not achieved the best results. In particular, adding $S3$ to the training phase harmed the performance of every classifier in comparison with using only $S1$ and $S2$. Recall that $S3$ contains only official Facebook political ads, and the performance of the classifier degraded probably because the characteristics of such ads are very different from the ones our system is expected to see in production ($S2$).

%Thus, considering all the possible combinations among $S1$, $S2$ and $S3$, as an effort to identify the best approach for our system, we observe that configurations using \update{$S1$ and $S2$}, yielded the best Macro-F1 scores. In particular, the CNN classifier with \update{$S1$ and $S2$} with text from $S2$ images is the one that achieved the best average result, with Macro-F1 \update{0.76} \update{($\pm0.06$) as shown on Table \ref{tab:text_and_images}. Adding text from $S2$ images on train improved our CNN model in $3\%$}. In fact, the CNN classifier was regularly the best method considering different sets of inputs. Also, note the increase in the Precision (\textbf{P}) scores for the political ads when $S2$ is added in the training phase of the model. This happened because $S1$ contains a set of political and non-political tweets posted by congressmen, which are helping the classifier to identify those political ads that are more subtle than traditional ``vote for Smith'' types of ads.


% \begingroup
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.0} % Default value: 1


% \endgroup
% \twocolumn

%Given these results, we have deployed three experimental versions of the system, each one deploying one of the models statistically tied as the best option. Three researchers individually evaluated these versions of the systems and unanimously preferred the model trained with Thus, we deployed the model trained with \update{$S1+S2$ and text extracted from $S2$ images} in our system.


\begin{table*}[t]
  
  \centering
  \caption{\update{Overall experiments results.}}
  
  \label{tab:result_table}
    \begin{tabular}{|c|r|c|c|c|c|c|c|c|c|c}
    	
    \hline
    \multirow{2}[2]{*}{} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Classifier}}} & \multirow{2}[2]{*}{\textbf{Accuracy}} & \multicolumn{3}{c|}{\textbf{Political}} & \multicolumn{3}{c|}{\textbf{Non Political}} & \multirow{2}[2]{*}{\textbf{Macro-F1}} \\
    
          & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \\

 & \multicolumn{1}{l|}{rforest} & $0.92 (\pm 0.008)$ & $0.95 (\pm 0.013)$ & $0.89 (\pm 0.013)$ & $0.92 (\pm 0.009)$ & $0.89 (\pm 0.013)$ & $0.95 (\pm 0.011)$ & $0.92 (\pm 0.008)$ & $0.92 (\pm 0.008)$ \\
 & \multicolumn{1}{l|}{logistic} & $0.94 (\pm 0.009)$ & $0.94 (\pm 0.018)$ & $0.95 (\pm 0.010)$ & $0.95 (\pm 0.010)$ & $0.95 (\pm 0.011)$ & $0.94 (\pm 0.019)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.009)$ \\
 & \multicolumn{1}{l|}{svm} & $0.94 (\pm 0.012)$ & $0.94 (\pm 0.019)$ & $0.95 (\pm 0.011)$ & $0.95 (\pm 0.011)$ & $0.95 (\pm 0.012)$ & $0.93 (\pm 0.020)$ & $0.94 (\pm 0.012)$ & $0.94 (\pm 0.012)$ \\
 & \multicolumn{1}{l|}{CNN} & $0.94 (\pm 0.010)$ & $0.97 (\pm 0.015)$ & $0.91 (\pm 0.027)$ & $0.94 (\pm 0.010)$ & $0.91 (\pm 0.027)$ & $0.97 (\pm 0.014)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.010)$ \\
 & \multicolumn{1}{l|}{NB} & $0.94 (\pm 0.009)$ & $0.91 (\pm 0.016)$ & $0.99 (\pm 0.006)$ & $0.95 (\pm 0.008)$ & $0.98 (\pm 0.007)$ & $0.90 (\pm 0.018)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.009)$ \\
 & \multicolumn{1}{l|}{gboosting} & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.017)$ & $0.92 (\pm 0.014)$ & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.015)$ & $0.92 (\pm 0.017)$ & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.011)$ \\
 
 \hline
    \end{tabular}%
  \label{tab:text_and_images}%
  
  
\end{table*}%

==> backup-4-classifier.tex <==
\section{Detecting political ads} \label{sec:methodology}

 In this section we describe our approach to identify political ads. This approach has three steps. First, we create a gold standard collection of ads used to test our method. Then, we select a supervised classifier that receives as input the text of an ad and outputs if it is political or non-political. Finally, we evaluate this classifier over different sets of training data.

\subsection{Gold Standard Collection}\label{sec:labeling-ads}

 To appropriately train and test our model, we needed a dataset with the same statistical properties as the ones we find in production, i.e., when the system goes online. The \textit{Official Political Facebook Ads} contains only political ads and the \textit{Twitter dataset} does not contain any ad, only tweets. Thus, we construct our \textit{gold standard collection} from the \textit{AdAnalyst dataset}, as the amount of political and non-political adds are distributed according to what users see in their feeds.

 From the $239K$ unique ads of this dataset, we sampled $10,000$ to be labeled by three independent volunteers. Their job is to label each ad of this sample as \textit{political} or \textit{non-political} according to Definition~\ref{def1}. We evaluate the inter-rater reliability among the independent volunteers  using the agreement percentage and the Cohen's Kappa coefficient ($\kappa$)~\cite{Oren2011,Landis1977,Savage2015}. This coefficient measures the agreement between two volunteers who each classify a predefined number of ads as one of the two mutually exclusive categories: \emph{political} or \emph{non-political}.

 From Table ~\ref{tab:labeled}, we observe that the agreement among the three volunteers is consistently high, 99.7\% for volunteers  1 and 2, with $\kappa = 0.93$, and 99.5\% for volunteers 1 and 3, with $\kappa = 0.88$. For volunteers 2 and 3 the agreement is 99.5\%, with $\kappa = 0.89$. According to Landis and Koch~\cite{Landis1977}, these Kappa scores fall into the range of scores referred to as ``Almost Perfect'' agreement, which is a satisfactory result that validates our \textit{gold standard collection}.

\begin{table}[ht]
\centering
\caption{Cohen's Kappa and Agreement percentage among researchers over \textit{labeled training set} containing $10,000$ Facebook ADs}

\label{tab:labeled}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
 & & \textbf{Researchers} \\
\hline
	&	\textbf{1 and 2}	&	\textbf{1 and 3} & \textbf{ 2 and 3} \\
\hline
Kappa coefficient $\kappa$	&	0.93	&	0.88	&   0.89 \\ 
Agreement \%			&	99.7\%	&	99.5\%  &   99.5\% \\
\hline
\end{tabular}
}
\end{table}

\subsection{Learning algorithms for automated detection of political ads}

 In a recent effort, Oliveira et al.~\cite{oliveira2018} proposed a successful Convolution Neural Network (CNN) architecture for identifying political tweets posted by politicians. Because of the similarity of their task with ours, we propose the use of the same architecture to identify political ads.

 Figure~\ref{fig:cnn_model} shows this architecture. In the input layer, we represent each word of a Facebook ad as a dense vector retrieved from Word2Vec C-BoW~\cite{Mikolov2013} with 300 dimensions, pre-trained over a large Portuguese data set \cite{Hartmann2017}, which is able to produce an embedding matrix for a vocabulary of 1.3 trillion words.
Thus, the input layer is a matrix $n \times 300$, where $n$ is the number of words in a particular ad and $300$ is the vector representation of each word of this message. Subsequently, there is a 25\% rate dropout regularization layer connected to a convolutional layer with $120$ different filters and sizes (3,4,5), activated by a ReLU function. Then, the output of the previous layer is connected to a global max-polling layer, whose output is, in turn, fully connected to a ReLU activation and to another 25\% rate dropout layer. Finally, the last dense layer is a single neuron with a sigmoid activation function that outputs $1$ if the message is \textit{political}, and $0$ if \textit{non-political}. Moreover, we optimized the neural network by means of cross entropy loss function using the RMSProp~\cite{Duchi2011} optimization algorithm.
 

\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\linewidth]{figures/cnn_model.pdf}
\caption{Convolutional Neural Network architecture for political Ads classification.}
\label{fig:cnn_model}
\end{figure*}
 
\subsection{Evaluation}

 \update{Our \textit{gold standard collection}, contains $233$ political and $9,767$ non-political advertisements manually labeled. In addition to this collection, we consider the another dataset described in Section~\ref{sec:dataset} for gathering textual features used to train and test our models:  the \textit{Official Political Facebook ads}, whose we randomly selected $10,000$ official political ads. Then, our train and test dataset has $20,000$ ads splitted in 10-\emph{folds}, $90\%$ for train and $10\%$ for test. In order to evaluate our choice of the classifier, we also run the results for four classic supervised baselines: Logistic Regression, Gradient Boosting, and Naive Bayes.}
 
 \update{In order to add extra textual feature to Lebaled Ads, we extracted texts from the all image in Labeled Ads, then we added to train. Our main goal adding these extra feature is investigated whether the model performance would be better than previous analysis without ad image features. In total, $7,598$ out of $10,000$ labeled ads had text. }

\if 0
\begin{table}[ht]
\small
  \caption{Text features for training and validation}
  \label{tab:features}
  \begin{tabular}{clccc}
    \toprule
    
    \textbf{Abbrv} & \textbf{Text feature} & \textbf{pol.} & \textbf{non-pol.} & \textbf{Total}\\
	
    \toprule
    $S1$ & Labeled Tweets  & $1,000$ & $1,000$ & $2,000$\\
    $S2$ & Labeled Facebook Ads & 233 & 9,767 & 10,000\\
    $S3$ & Official Political Facebook Ads\footnote{https://www.facebook.com/politicalcontentads} & \update{26,059} & 0 & \update{26,059}\\
  \bottomrule
\end{tabular}
\end{table}
\fi

As evaluation metrics, we considered two classic metrics: accuracy and Macro-F1. Accuracy considers equally important the correct classification of each ad, independently of the class, and basically measures the capability of the method to predict the correct output. A variation of F1, namely, Macro-F1, is normally reported to evaluate classification effectiveness on skewed
datasets.  Macro-F1 values are computed by first calculating F1 (a metric that captures both precision and recall) values for each class in isolation, then averaging over all classes. This way, Macro-F1 considers equally important the effectiveness in each class, independently of the relative
size of the class.

%In the training process we used $10$\emph{-fold} \emph{cross-validation}. 
%For each test fold $i$, we trained the model with the rest, until all folds have been used as test fold. Then, we calculate the mean and confidence interval for each class metrics (\emph{precision}, \emph{recall}, \emph{f1}), also \emph{Macro-F1}, \emph{AUC - Area Under the Roc Curve}  and \emph{accuracy}. 


\begin{table}[ht]
\centering
\tiny
\caption{Results obtained for different classifiers w.r.t
AUC and F1-macro score}

\label{tab:results_experiments}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\hline
 & \textbf{Metrics} &  \\
\hline
	&	\textbf{AUC}	&	\textbf{F1-macro}  \\
\hline
CNN 	        & $0.98 (\pm 0.010)$	& $0.94 (\pm 0.010)$ \\ 
SVM 			& $0.98 (\pm 0.010)$  & $0.94 (\pm 0.012)$ \\
L. Regression 	& $0.98 (\pm 0.014)$  & $0.94 (\pm 0.009)$ \\
R. Forest 		& $0.97 (\pm 0.012)$	& $0.92 (\pm 0.008)$ \\
N. Bayes 		& $0.99 (\pm 0.011)$  & $0.94 (\pm 0.009)$ \\
G. Boosting 	&$0.97 (\pm 0.019)$	& $0.92 (\pm 0.011)$ \\

\hline
\end{tabular}
}
\end{table}

%Also, we evaluate the classification performance of the each learning method considering each combination of textual features as input: $S1$, $S2$, $S3$, $S1 + S2$, $S1 + S3$, $S2 + S3$, $S1 + S2 + S3$. Our goal is to assess the discriminating power of adding each set of textual features and understand if adding features from tweets, for example, would add noise or help in differentiate political ads from the non-political ones.

%In Table~\ref{tab:tabelao2}, we show the results for all configurations of \textbf{input} and \textbf{method}. We highlight in bold all the configurations that achieved the statistically highest Macro-F1 scores. First, observe that using all datasets as input have not achieved the best results. In particular, adding $S3$ to the training phase harmed the performance of every classifier in comparison with using only $S1$ and $S2$. Recall that $S3$ contains only official Facebook political ads, and the performance of the classifier degraded probably because the characteristics of such ads are very different from the ones our system is expected to see in production ($S2$).

%Thus, considering all the possible combinations among $S1$, $S2$ and $S3$, as an effort to identify the best approach for our system, we observe that configurations using \update{$S1$ and $S2$}, yielded the best Macro-F1 scores. In particular, the CNN classifier with \update{$S1$ and $S2$} with text from $S2$ images is the one that achieved the best average result, with Macro-F1 \update{0.76} \update{($\pm0.06$) as shown on Table \ref{tab:text_and_images}. Adding text from $S2$ images on train improved our CNN model in $3\%$}. In fact, the CNN classifier was regularly the best method considering different sets of inputs. Also, note the increase in the Precision (\textbf{P}) scores for the political ads when $S2$ is added in the training phase of the model. This happened because $S1$ contains a set of political and non-political tweets posted by congressmen, which are helping the classifier to identify those political ads that are more subtle than traditional ``vote for Smith'' types of ads.


% \begingroup
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.0} % Default value: 1


% \endgroup
% \twocolumn

%Given these results, we have deployed three experimental versions of the system, each one deploying one of the models statistically tied as the best option. Three researchers individually evaluated these versions of the systems and unanimously preferred the model trained with Thus, we deployed the model trained with \update{$S1+S2$ and text extracted from $S2$ images} in our system.


\begin{table*}[t]
  
  \centering
  \caption{\update{Overall experiments results.}}
  
  \label{tab:result_table}
    \begin{tabular}{|c|r|c|c|c|c|c|c|c|c|c}
    	
    \hline
    \multirow{2}[2]{*}{} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Classifier}}} & \multirow{2}[2]{*}{\textbf{Accuracy}} & \multicolumn{3}{c|}{\textbf{Political}} & \multicolumn{3}{c|}{\textbf{Non Political}} & \multirow{2}[2]{*}{\textbf{Macro-F1}} \\
    
          & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \textbf{F1} & \\

 & \multicolumn{1}{l|}{rforest} & $0.92 (\pm 0.008)$ & $0.95 (\pm 0.013)$ & $0.89 (\pm 0.013)$ & $0.92 (\pm 0.009)$ & $0.89 (\pm 0.013)$ & $0.95 (\pm 0.011)$ & $0.92 (\pm 0.008)$ & $0.92 (\pm 0.008)$ \\
 & \multicolumn{1}{l|}{logistic} & $0.94 (\pm 0.009)$ & $0.94 (\pm 0.018)$ & $0.95 (\pm 0.010)$ & $0.95 (\pm 0.010)$ & $0.95 (\pm 0.011)$ & $0.94 (\pm 0.019)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.009)$ \\
 & \multicolumn{1}{l|}{svm} & $0.94 (\pm 0.012)$ & $0.94 (\pm 0.019)$ & $0.95 (\pm 0.011)$ & $0.95 (\pm 0.011)$ & $0.95 (\pm 0.012)$ & $0.93 (\pm 0.020)$ & $0.94 (\pm 0.012)$ & $0.94 (\pm 0.012)$ \\
 & \multicolumn{1}{l|}{CNN} & $0.94 (\pm 0.010)$ & $0.97 (\pm 0.015)$ & $0.91 (\pm 0.027)$ & $0.94 (\pm 0.010)$ & $0.91 (\pm 0.027)$ & $0.97 (\pm 0.014)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.010)$ \\
 & \multicolumn{1}{l|}{NB} & $0.94 (\pm 0.009)$ & $0.91 (\pm 0.016)$ & $0.99 (\pm 0.006)$ & $0.95 (\pm 0.008)$ & $0.98 (\pm 0.007)$ & $0.90 (\pm 0.018)$ & $0.94 (\pm 0.010)$ & $0.94 (\pm 0.009)$ \\
 & \multicolumn{1}{l|}{gboosting} & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.017)$ & $0.92 (\pm 0.014)$ & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.015)$ & $0.92 (\pm 0.017)$ & $0.92 (\pm 0.011)$ & $0.92 (\pm 0.011)$ \\
 
 \hline
    \end{tabular}%
  \label{tab:text_and_images}%
  
  
\end{table*}%
